Segmental Spatiotemporal CNNs for Fine-grained Action Segmentation

Joint segmentation and classification of fine-grained actions is important for applications of human-robot interaction, video surveillance, and human skill evaluation. However, despite substantial recent progress in large-scale action classification, the performance of state-of-the-art fine-grained action recognition approaches remains low. We propose a model for action segmentation which combines low-level spatiotemporal features with a high-level segmental classifier. Our spatiotemporal CNN is comprised of a spatial component that uses convolutional filters to capture information about objects and their relationships, and a temporal component that uses large 1D convolutional filters to capture information about how object relationships change across time. These features are used in tandem with a semi-Markov model that models transitions from one action to another. We introduce an efficient constrained segmental inference algorithm for this model that is orders of magnitude faster than the current approach. We highlight the effectiveness of our Segmental Spatiotemporal CNN on cooking and surgical action datasets for which we observe substantially improved performance relative to recent baseline methods.

==> IEEEtranBST/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

IEEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> sections/data.tex <==
\section{Data}
\label{sec:data}




==> sections/discussion_old.tex <==
\section{Discussion}
\label{sec:discussion}

The results in Tables~\ref{table:salads} and \ref{table:jigsaws} are consistent with our hypothesis that holistic methods like IDT are insufficient for fine-grained action segmentation. Regardless of the temporal model, performance of our CNN-based scene model is superior to the IDT baselines.

Many actions in 50 Salads, like cutting, require capturing small hand motions. We visualized IDT
\footnote{Visualization was performed using the public software from Wang \etal \cite{wang_iccv_2013}.}
and found it does not detect many tracklets for these actions. To contrast, large-motion actions like placing ingredients in the bowl generate thousands of tracklets. Performance is negatively effected even when compensating for the imbalance by normalizing feature histograms. We visualized our method, for example as shown in Figure~\ref{fig:activations}, and qualitatively found it is better at capturing details necessary for finer actions. 


Based on ablative analysis of our model we see that each component makes an important contribution. 
The spatiotemporal model (\textit{Scene+Evo}) outperforms the spatial model (\textit{Scene}) by 29\% accuracy on JIGSAWS and 4.7\% on 50 Salads using the ``eval" granularity. The large effect on JIGSAWS may be contributed to the fact that there is less visual variation in each of the actions. For example both \textit{transfer tool} and \textit{insert needle into skin} can appear in the center of the screen. However, the tools start and end in different locations for each action. Results on both datasets improve tremendously in terms of edit distance. Figure~\ref{fig:timeline} shows that the predictions using just the \textit{Scene} model tends to oscillate over time compared to the improved models. 

Adding the segmental model has a large impact on the edit score of all tested models. In many cases edit performance improves by 10\%. For example on JIGSAWS the \textit{Scene+Evo} model achieves 71.23\% and \textit{Scene+Evo+Seg} achieves 82.16\%. Interestingly, in most cases the accuracy between frame-wise and segmental does not vary significantly. This implies that the percent of frames that are correct is roughly constant but the number of false-positives decreases. This is important for robotics applications where false-positives can be especially problematic. \TODO{elaborate}

\begin{figure*}[tb]
  \includegraphics[width=\hsize]{imgs/timeline}
  \caption{The plots on top depict the ground truth action predictions for a given video. Each color corresponds to a different class label. The second row, sCNN, depicts the predictions using the spatial component of our model. The third row, stCNN, depicts predictions using the spatiotemporal model with frame-wise inference. The bottom row uses the spatiotemporal model with segmental inference.}
  \label{fig:timeline}
\end{figure*}


%In all experiments the video results are strictly worse than sensor results in terms of accuracy. This is not surprising given that the sensors were specifically designed to model each activity. For example in 50 Salads the accelerometers are attached to a kitchen utensil that corresponds to one of the ``eval" labels. In JIGSAWS the robot pose includes the 3D position and orientation of the robot tools as well as whether or not the grippers are closed. From our spatial activation maps (as shown in Section~\ref{sec:model}) we see that our model detects the positions of the tools. However, it is unclear if it is picking up on depth information. If we used stereo images then perhaps we could improve performance. 

%We were surprised to find that despite the video accuracy being lower, the segmental scores are very similar those using sensor data. This implies that the sensor-based approaches tend to have more false positives. It is unclear what causes this.

Table~\ref{table:granularities} shows results for each granularity of 50 Salads. 
%While the performance decreases going from ``high" to ``low" the difference in sensor accuracies for ``medium" (18 classes) compared to ``low" (52 action classes) is relatively small. 
While performance decreases as the number of classes increases, results degrade sub-linearly with each additional class. 
The classification scores are modest. This is in large part due to the background class. There are many very short background actions that happen in between other long segments. Our model does not recognize these well which has a large impact on classification accuracy. \TODO{recompute without background class}

%There are a small number of instances with the accelerometer data when most of the devices would activate simultaenously. This cause some errors in prediction.  We think this may have happend if, for example, the table was bumped. This is one drawback to using these sensors 

Figure~\ref{fig:confusion} depicts the confusion matrix for the ``low" granularity on 50 Salads\footnote{A larger version of this appears in the supplemental material.}. The white boxes overlaid denote which ``low" level actions correspond to which object-agnostic actions. 
For example all \textit{cutting} actions are in one box. As expected the highest errors for each action are within that box. The method tends to confuse \textit{cutting a tomato} with \textit{cutting a cucumber} more than it confuses it with \textit{mixing ingredients}. 
% It also tends to get the start, middle, and end of each action confused more than with other actions. 

Overall the video results on JIGSAWS have 4.1\% higher accuracy relative to the state of the art~\cite{tao_miccai_2013} which uses a holistic approach.
%Our sensor results have a 7.5\% relative increase in the segmental score than~\cite{lea_icra_2016} but 5.1\% decrease in accuracy. 
Our classification accuracy on JIGSAWS using video is 90.47\%. This is notably higher than the state of the art \cite{zappella_media_2013} which achieves 81.17\%. 
% and using sensors is 86.63\%. 
% Both of these are slightly higher than state of the art which is 81.17\% for video and 86.56\% for sensor data \cite{zappella_media_2013}. 


\begin{figure}
	\center
	\includegraphics[width=.5\hsize]{imgs/confusion_mat/low}
	\caption{Confusion matrix for the ``low" granularity in the 50 Salads dataset. A higher resolution image is included in the supplemental material.}
	\label{fig:confusion}
\end{figure}


The speedup of our algorithm compared to Segmental Viterbi is shown in Table~\ref{table:speedup}.
One practical implication is that our algorithm scales readily to full-length videos. 
On 50 Salads, Segmental Viterbi takes 2 hours to compute high-level predictions for all trials compared to a mere 4 seconds using ours. In addition, we explicitly store the score for each segment and frame thus  the resulting score table is easier to interpret and analyze.



LSTM versus Evo.

%The speedup here could enable new work on hierarchical models.
% like proposed (but not implemented) in~\cite{pirsiavash_cvpr_2014}. 
%Given our performance boost and speed increases we hope to see others adopt this method in future work. 




%\textbf{50 Salads:}
%We are not aware of any other video-based results on 50 Salads and thus can only compare against the sensor-based results. The  

% ICRA They use a temporal model that shares similarities to our temporal model but is defi
%similar to our temporal that is conceptually similar

%\textbf{LSTM}


%It is important for many practical applications that we reduce the number of these false positives, hence why the segmental edit distance is a good metric.
%\TODO{mention slight temporal deviations}
% These false-positives do not substantially impact the frame-wise accuracy because they are short in duration, however, for it is important to reduce them in practical applications. 

%While the results using our video-based approach are not as high as the results from the domain-specifc sensors, they are approaching that performance. 


%Figure~\ref{fig:weights} depicts a representative sample of the temporal filters learned from our model in the ``low" granularity regime in 50 Salads. The $x$-axis corresponds to filter duration and the $y$-axis corresponds to features. Most filters have a small set of features with very high weights (red) for a large period of time, a small set of weights with very negative (blue) weights, and most features with neglible weight (green). A small number of the filters, like the left-most one in the figure, do not have a coherent structure. 

%\begin{figure}
%\center
%	\includegraphics[width=.99\hsize]{imgs/weights}
%	\caption{Example filters learned from the 50 Salads dataset using the temporal component of our model. Each filter duration is 100 timesteps.}
%	\label{fig:weights}
%\end{figure}



%* tried hierarchy of temporal filters. didn’t help. think it has to do with learning duration of actions




%Issues with inference:
%\begin{figure}
%\center
%	\includegraphics[width=.6\hsize]{imgs/tmp}
%	\caption{Inference issues in segmental models}
%	\label{fig:sm-inference}
%\end{figure}


%We performed preliminary experiments using a pre-trained VGG~\cite{VGG} and Alexnet~\cite{Alexnet} networks. We found that the performance was much lower than when using our networks trained on this data. We believe there are two reasons for this. First, the pre-trained networks were learned on Imagenet which has very different kinds of objects than in our data. They are trying to differentiate between distinct classes like cats and cars whereas we are trying to distinguish between more fine-grained objects. Second, their networks try to be spatially-invariant so that an object is classified correctly regardless of were it is in the image. In our case we want to retain spatial information; if a user's hand is in the bottom-left of the image it may mean something else semantically than if it is in the top-right. Furthermore the grid size used in these models is finer than what we have found is appropriate for our tasks. 

%We found that typical methods for data augmentation, such as shifting each image, provided worse results. This is not unexpected given that the locations of objects in the scene is important; shifting the images causes the absolute location of each object to move. Furthermore, our data was recorded at 30 frames per second. Thus we get many slight variations of an action for free. \TODO{remove first part; it feels out of place. The last part is interesting though!}



% blah; We highly suggest using the Salads dataset for further work in this area. It has the following benefits over other datas (tested here and elsewhere): (1) lots of samples (2) semi-structured (3) multiple levels of labels [can start with research on high level actions… then work your way to harder, more fined grained ones] (4) multi-modal (5) …


==> sections/evaluation_Conflict_.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section we introduce our datasets, metrics, and results on the University of Dundee 50 Salads dataset~\cite{stein_ubicomp_2013} and the JHU-ISI Gesture and Skills Assessment Working Set (JIGSAWS)~\cite{jigsaws-m2cai}. While 50 Salads was developed by researchers in the ubiquitous computing community, we believe it provides great value to the computer vision community due to the large number of action instances per class, the high quality labels, plethora of data, and multi-modal sensors. This dataset can be used to answer many research questions regarding fine-grained action analysis. 

\TODO{uncomment comparison with other datasets?}
%Many current fine-grained action recognition datasets are limited by size. The MPII Cooking dataset is offers a realistic cooking environment and many different activities, however, many action labels are rarely used. For example, 7 actions (of \TODO{64?} are performed less than 10 times. Similarly, the Georgia Tech Egocentric Activities dataset is nice because if has 7 unique tasks, however, but there are only 3 users to test on and one for evaluation. 


%In this section we discuss the two datasets, our evaluation metrics, and experiments using our models. 

%We perform a comprehensive set of experiments to show ablative analysis, the effect of training on different action granularities,
%and how our model performs if we assume temporal segmentation. Note that our emphasis is not on how the accuracy alone improves, but on how well the segments are modeled. For many applications having a set of cohesive segments is at least, if not more, important than good accuracy. 


%We perform a set of experiments: (1) How does each component of our model (spatial, spatial-temporal, segmental) contribute to overall performance? (2) How does using finer- versus coarser-grained action labels impact performance? (3) Does performance change if we train with a set of finer-grained set of labels than we need? (4) Can we train on one fine-grained dataset and test on another in a different domain? (5) How does our model perform if we have known temporal segmentation? \TODO{say this in words}

%\TODO{reference ICRA paper}

\subsection{University of Dundee 50 Salads}
Stein and McKenna introduced 50 Salads \cite{stein_ubicomp_2013} for evaluating fine-grained action recognition in the cooking domain. This dataset includes 50 instances salad preparation. Each of the 25 users makes a salad in two different trials. Trials include video, depth maps (via Kinect), and synchronized 3-axis accelerometer data from 10 kitchen objects. These accelerometers can be used as a proxy for which objects are being used in the scene. The objects are: \textit{plate}, \textit{pepper dispenser}, \textit{bowl}, \textit{oil bottle}, \textit{large spoon}, \textit{dressing glass}, \textit{knife}, \textit{peeler}, \textit{small spoon}, and \textit{chopping board}.

Videos are annotated at four levels of granularity. The coarsest level (``high'') consists of labels \textit{cut and mix ingredients}, \textit{prepare dressing}, and \textit{serve salad.}. At the second tier (``mid'') there are 17 fine-grained actions like \textit{add vinegar}, \textit{cut tomato}, \textit{mix dressing}, \textit{peel cucumber}, \textit{place cheese into bowl}, \textit{serve salad} and others. At the finest level (``low'') there are 51 actions indicating the start, middle, and end of the previous 17 actions. For each level there is also a \textit{background} class. All actions are listed in the supplemental material. 

%The second granularity (``eval") adds object-agnostic actions like \textit{cutting} 
%%consolidates object-specific actions like \textit{cutting a tomato} and \textit{cutting a cucumber} into a . 
%%For example instead of having a separate action for \textit{cutting a cucumber} and \textit{cutting cheese} there is a single \textit{cutting} action. 
%These actions are: \textit{add dressing, add oil, add pepper, cut, mix dressing, mix ingredients, peel, place} and \textit{serve salad}.

A fourth granularity (``eval"), suggested by \cite{stein_ubicomp_2013}, consolidates some object-specific actions like \textit{cutting a tomato} and \textit{cutting a cucumber} into object-agnostic actions like \textit{cutting}.
%For example instead of having a separate action for \textit{cutting a cucumber} and \textit{cutting cheese} there is a single \textit{cutting} action. 
Actions include \textit{add dressing}, \textit{add oil}, \textit{add pepper}, \textit{cut}, \textit{mix dressing}, \textit{mix ingredients}, \textit{peel}, \textit{place}, \textit{serve salad on plate}, and \textit{background}. These labels coincide with the tools instrumented with accelerometers.

%Our sensor-based results use the same features as \cite{Lea_icra_2016} which are the absolute value of the accelerometer values. We use the same splits with 5-fold validation where we train on 20 users and test on 5 users.

%\subsubsection{50 Salads}
%50 Salads \cite{Stein_2013b} is a multimodal dataset that includes time-synchronized video, depth, and accelerometer data. There are 50 five- to 10-minute samples of a user making a salad. In total there are 25 users -- each of whom makes a salad in two different videos. As shown in figure~ref{fig:salads} a static RGBD camera is mounted facing down looking at the user preparing the salad. Each kitchen utensil has an accelerometer attached that records motion. These can be used to indicate which tools is being used at any given time. In total there are 10 accelerometers. These are located on the following kitchen tools: \textit{plate, pepper\_dispenser, bowl, oil\_bottle, large\_spoon, dressing\_glass, knife, peeler, small\_spoon, chopping\_board}.
%
%One novelty of this dataset is that there are multiple granularities of action labels. At the coarsest there are three actions: \textit{cut\_and\_mix\_ingredients, prepare\_dressing, serve\_salad.} At the most fine-grain it has labels for the start, core, and end of 17 different action primitives such as \textit{add\_vinegar, cut\_tomato, mix\_dressing, peel\_cucumber, place\_cheese\_into\_bowl, serve\_salad.} Following the work of \cite{Stein_2013,Stein_2013b,Yang_Humanoids_2014}, we use the following set of 10 labels for this paper: \textit{add\_dressing, add\_oil, add\_pepper, cut, mix\_dressing, mix\_ingredients, peel, place, serve\_salad\_onto\_plate}. This is a set of hybrid labels that combines types of cutting and placing actions.
%
%In our experiment we only use the accelerometer data. It is reasonable to assume that we could learn object detectors for each of the tools which could be used in place of the accelerometers for purely vision-based applications. 
%
%We evaluate on use the set of 10 action labels from \cite{Stein_2013b}.
%\TODO{ the other relevant papers:} \cite{Stein_2013,Stein_2013b,Yang_Humanoids_2014}

\subsection{JHU-ISI Gesture and Skill Assessment Working Set (JIGSAWS)}
The second dataset, JIGSAWS \cite{jigsaws-m2cai}, is used for recognizing fine-grained actions common in robotic surgery training. We use Leave One User Out evaluation on the suturing task. This includes 39 trials of synchronized video and robot kinematics data collected from a daVinci medical robot. There are eight users and about five trials per user. Each trial is decomposed into 11 fine-grained actions such as \textit{inserting\_needle\_into\_skin, tying\_a\_knot, transferring\_needle\_between\_tools}, and \textit{dropping\_the\_needle\_at\_the\_end\_point.}  Videos last about two minutes and contain 15 to 37 action primitives per video.

\TODO{more details? mention lingling's paper}
%In the sensor-based baseline we use the robot kinematics and vision-based features from the authors of \cite{lea_wacv_2015}. The features are: left and right tool positions, velocities, and gripper angles as well as the distance from the tools to the closest object in the scene from the video.

%------------------------------------------------------------------------------------
\subsection{Metrics}
We evaluate on two metrics: one that measures how well segments are captured and the other that measures the framewise accuracy of the predictions.

First, we use the Levenshtein edit distance as a segmental metric. This metric was suggested for the 50 Salads dataset by \cite{Lea_icra_2016} because it penalizes oversegmentation but allows for slight temporal deviations between the ground truth and predictions. In many applications there is high uncertainty in the location of temporal boundaries. The start or end of an action may be ambiguous or different annotators may interpret an action differently.

This score, $A_{edit}(G,P)$, is computed as a function of segment insertions, deletions, with ground truth segments $G=\{G_1,\dots, G_M\}$ and predicted segments $P=\{P_1,\dots, P_N \}$. The number of edits is normalized by the maximum of $M$ and $N$. For clarity we show the score $(1-A_{edit}(G,P)) \times 100 $ which is a number from 0 to 100. 

%We compute the normalized Levenshtein edit distance $A_{edit}(G',P')$ using the Wagner-Fischer algorithm which penalizes segment insertions, deletions, and substitutions. 

In order to compare against prior work we also evaluate using framewise accuracy. Let $G=\{y_1,\dots,y_T\}$ be ground truth labels at each timestep and $P=\{y_1,\dots,y_T\}$ be the predicted labels. Framewise accuracy captures the percent of time a class is correctly classified: $A_{acc}(G,P)=\frac{1}{T} \sum_{t=1}^T \mathbf{1}(G_t=P_t)$. The classification results, which assume temporal segmentation, use the accuracy metric applied to segments instead of individual frames.

%measures the overlap between ground truth and predicted segments. It is especially important for applications in human-robot collaboration. 
%This metric is similar to a Jaccard Index but penalizes for gratuitous oversegmentation, such as those resulting from oscillations in action predictions. %This score ranges from 0 to 100 and a higher score is better. 


%The second metric accounts for slight temporal shifts in the prediction. In many domains there is large inter-annotator variability in labeling where temporal boundaries should be located. In applications like surgical skill evaluation the ordering of the actions may matter more than the precise location of the segments. 
%To measure this error we use a segmental edit score. For each ground truth and predicted labeling we first output the sequence of actions (independent of segmentation boundaries). We then compute a normalized edit distance, $s_e(G,P)$, using the Wagner-Fischer algorithm. To make it easier to interpret the results we show scores for $(1-s_e(G,P))*100$. The best score 100 and the worst is 0.

%Note that for convenience in interpreting the results we normalize this score using the length of the ground truth sequence. The best score is 0 and it is unbounded from above. A lower score is better.


%------Metrics when I was planning on using the overlap score----
%%------------------------------------------------------------------------------------
%\subsection{Metrics}
%\THOUGHT{use the segmental edit distance instead. it shows larger discrepancy in segmental model}
%We compute two evaluation metrics: framewise accuracy and a segment-level overlap function. The segmental method was proposed by \cite{ICRA} and measures the overlap between ground truth and predicted segments. It is especially important for applications in human-robot collaboration. 
%This metric is similar to a Jaccard Index but penalizes for gratuitous oversegmentation, such as those resulting from oscillations in action predictions. Given a ground truth sequence $G$ and predicted sequence $P$ the score is:
%\begin{equation}
%A(G, P) = \frac{100}{N} \sum_{i=1}^M \max_j \frac{G_i \cap P_j}{G_i \cup P_j}
%\end{equation}
%This score ranges from 0 to 100 and a higher score is better. 
%
%%The first score measures how much overlap there is between the ground truth segments and the predicted segments. A common metric for this is the Jaccard Index. While this does a good job at measuring coverage, it does not penalize for oversegmentation errors. Predictions from models like the Skip Chain CRF will sometimes add spurious false labels within what should be a long contiguous segment. We penalize these errors by defining an overlap score that is a function of the longest contiguous predicted segment for a given ground truth segment. 
%
%%The second metric accounts for slight temporal shifts in the prediction. In many domains there is large inter-annotator variability in labeling where temporal boundaries should be located. In applications like surgical skill evaluation the ordering of the actions may matter more than the precise location of the segments. To measure this error we use a segmental edit score. For each ground truth and predicted labeling we first output the sequence of actions (independent of segmentation boundaries). We then compute a normalized edit distance, $s_e(G,P)$, using the Wagner-Fischer algorithm. To make it easier to interpret the results we show scores for $(1-s_e(G,P))*100$. The best score 100 and the worst is 0.
%
%%Note that for convenience in interpreting the results we normalize this score using the length of the ground truth sequence. The best score is 0 and it is unbounded from above. A lower score is better.
%
%%Accuracy 
%%Accuracy is the traditional way of measuring accuracy for activity recognition. It is computed as the mean of all correct frames: $m_i(y, y^*) = \frac{1}{N} \sum_{i=1}^N \delta(y_i, y_i^*) $ where $\delta$ is 1 if $y_i$ and $y_i^*$ are the same label and 0 otherwise. 
%
%%We also use accuracy, precision, and recall to compare against prior work. These are defined using $TP$, $FP$, $TN$, and $FN$ for true positives, false positives, true negatives, and false negatives.
%%\begin{align}
%%\text{Accuracy }&= \frac{TP+TN}{TP+FP+FN+TN} \\
%%\text{Precision }&= \frac{TP}{TP+FP}\\
%%\text{Recall }&= \frac{TP}{TP+FN}
%%\end{align}

%------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------
\subsection{Experiments}
%-------------------------------------------------------------
%-------------------------------------------------------------
In our first experiment, shown in Table~\ref{table:results1}, we compare our results with other work and perform an ablative analysis to show the performance using the spatial, the spatiotemporal, and the segmental spatiotemporal models. These 50 Salads results are on the ``eval" granularity.
%For clarity methods using sensor data are shown separately. 

We provide a matrix of experiments showing the effect of each spatial and temporal model. We evaluate using two spatial features: our CNN and a Dense Trajectory baseline. Furthermore, we use each set of spatial features as input into the temporal models. We have three temporal models: a Sliding SVM baseline, an RNN-LSTM baseline, our intra-action model, and our full model. 
%The Sliding SVM is comparable to Rohrbach \etal~\cite{rohrbach_ijcv_2015} where we use a sliding window of 30 frames.
The Sliding SVM is comparable to the only localization model submitted to the THUMOS 2015 action recognition competition \TODO{check}. 
The RNN-LSTM baseline uses one layer of LSTM units with 64 latent nodes. 

Our IDT baseline is comparable to Rohrbach \etal~\cite{rohrbach_ijcv_2015} on the MPII dataset. We extract IDT, create a KMeans dictonary (k=2000) on the HOG channel, and use a sliding window of 30 frames to compute a local histogram. As with \cite{sivic}, we found HOG alone performed better than HOG+HOF+MBH+Traj. Note that IDT features alone took 18 hours to compute on 50 Salads compared to 5 hours for our CNN features.
\TODO{mention our IDT results are comparable to Li on GTEA}

%we achieve 56.29\% accuracy on the 50 Salads ``eval'' set and 52.70\% on JIGSAWS.  
%We also experimented using the IDT-based frame-level features as input into our temporal CNN. We achieve 61.46\% and 72.10\% respectively on these datasets. 
%All IDT results are lower than from the full model in our paper.
%These results are consistent with findings of Li \etal (CVPR15) on the Georgia Tech Egocentric Activities dataset and in the CVPR2015 THUMOS action localization challenge. 
%While IDT are great for large-scale action classification, we found they do not capture nuances of fine-grained action segmentation and classification. 



%Our LSTM model 

%In addition to evaluating our model on video data, we compare performance of the temporal component (with and without segmental inference) using the sensor data from each dataset. We also evaluate these results using LSTM, a popular Recurrent Neural Network. In these results we use 64 latent nodes.


%\begin{table}
%\begin{center}
%\begin{tabular}{c}
%50 Salads\\
%% -----------Salads----------
%\begin{tabular}{| l | c | c |}
%%\hline
%%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
%% & Framewise & Segmental \\
%\hline
%\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy}\\
%\hline
%\cite{Lea_icra_2016} LC-SC-CRF & \textbf{58.08} & 81.75 \\
%LSTM (framewise) & 47.71 & 70.00\\ 
%LSTM (segmental)  & 51.25 & 69.80\\ 
%%CLF sensor lstm   & 46.62 & 49.28\\ 
%%\hline
%tCNN (framewise)  & 45.67 & 82.12\\ 
%tCNN (segmental) & 55.50 & \textbf{82.14} \\ 
%%CLF sensor   & 60.10 & 64.32\\ 
%\hline
%\textbf{Video-based} & \textbf{Edit} & \textbf{Accuracy} \\
%\hline
%sCNN (framewise)  & 24.10 & 66.64\\ 
%stCNN (framewise)  & 49.6 & 69.35\\ 
%stCNN (segmental)  &\textbf{55.96} & \textbf{69.36}\\ 
%%CLF  & 65.85 & 69.06\\ 
%\hline
%\end{tabular}
%\end{tabular}
%\end{center}
%\caption{ Results on 50 Salads and JIGSAWS.}
%\label{table:results1}
%\end{table}
%
%\begin{table}
%\begin{center}
%\begin{tabular}{c}
%JIGSAWS
%\\
%\begin{tabular}{| l | c | c |}
%%\hline
%%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
%\hline
%\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy} \\
%\hline 
%\cite{Stefati_m2cai_2015} SD-SDL & -  & 78.68 \\
%\cite{Lea_icra_2016} LC-SC-CRF & 76.86 & \textbf{83.45}  \\
%LSTM (framewise)  & 60.94 & 66.32\\ 
%LSTM (segmental)  & 68.96 & 65.60\\ 
%%CLF sensor lstm & 78.16 & 73.1 \\ 
%%\hline
%tCNN (framewise)  & 75.78 & 79.00\\ 
%tCNN (segmental)   & \textbf{82.63} & 79.17\\ 
%%CLF sensor   & 86.44 & 86.63\\ 
%\hline 
%\textbf{Vision-based }  & \textbf{Edit} & \textbf{Accuracy}\\
%\hline
%\cite{tao_miccai_2013} MsM-CRF  & -& 71.78 \\
%sCNN (framewise)  & 17.44 & 57.80\\ 
%stCNN (framewise)  & 71.23 & 74.59\\ 
%stCNN (segmental) &  \textbf{82.16} & \textbf{74.75}\\ 
%%CLF  & 83.87 & 83.39\\ 
%\hline
%\end{tabular}
%\end{tabular}
%\end{center}
%\caption{ Results on 50 Salads and JIGSAWS.}
%\label{table:results1}
%\end{table}


%\begin{table}
%\begin{center}
%\begin{tabular}{c}
%50 Salads\\
%% -----------Salads----------
%\begin{tabular}{| l | c | c |}
%%\hline
%%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
%% & Framewise & Segmental \\
%\hline
%\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy}\\
%\hline
%\cite{Lea_icra_2016} LC-SC-CRF & \textbf{58.08} & 81.75 \\
%LSTM (framewise) & 47.71 & 70.00\\ 
%LSTM (segmental)  & 51.25 & 69.80\\ 
%%CLF sensor lstm   & 46.62 & 49.28\\ 
%%\hline
%tCNN (framewise)  & 45.67 & 82.12\\ 
%tCNN (segmental) & 55.50 & \textbf{82.14} \\ 
%%CLF sensor   & 60.10 & 64.32\\ 
%\hline
%\textbf{Video-based} & \textbf{Edit} & \textbf{Accuracy} \\
%\hline
%sCNN (framewise)  & 24.10 & 66.64\\ 
%stCNN (framewise)  & 49.6 & 69.35\\ 
%stCNN (segmental)  &\textbf{55.96} & \textbf{69.36}\\ 
%%CLF  & 65.85 & 69.06\\ 
%\hline
%\end{tabular} \\
%\\
%JIGSAWS
%\\
%\begin{tabular}{| l | c | c |}
%%\hline
%%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
%\hline
%\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy} \\
%\hline 
%\cite{Stefati_m2cai_2015} SD-SDL & -  & 78.68 \\
%\cite{Lea_icra_2016} LC-SC-CRF & 76.86 & \textbf{83.45}  \\
%LSTM (framewise)  & 60.94 & 66.32\\ 
%LSTM (segmental)  & 68.96 & 65.60\\ 
%%CLF sensor lstm & 78.16 & 73.1 \\ 
%%\hline
%tCNN (framewise)  & 75.78 & 79.00\\ 
%tCNN (segmental)   & \textbf{82.63} & 79.17\\ 
%%CLF sensor   & 86.44 & 86.63\\ 
%\hline 
%\textbf{Vision-based }  & \textbf{Edit} & \textbf{Accuracy}\\
%\hline
%\cite{tao_miccai_2013} MsM-CRF  & -& 71.78 \\
%sCNN (framewise)  & 17.44 & 57.80\\ 
%stCNN (framewise)  & 71.23 & 74.59\\ 
%stCNN (segmental) &  \textbf{82.16} & \textbf{74.75}\\ 
%%CLF  & 83.87 & 83.39\\ 
%\hline
%\end{tabular}
%\end{tabular}
%\end{center}
%\caption{ Results on 50 Salads and JIGSAWS.}
%\label{table:results1}
%\end{table}

\begin{table}
%	\begin{center}
%		\begin{tabular}{c c}
%			50 Salads & JIGSAWS \\
			% -----------Salads----------
			\begin{minipage}[t]{0.5\linewidth}
			\begin{center}
				\textbf{50 Salads} \\
			\begin{tabular}{| l | c | c |}
				%\hline
				%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
				% & Framewise & Segmental \\
%				\hline
%				\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy}\\
%				\hline
%				\cite{Lea_icra_2016} LC-SC-CRF & \textbf{58.08} & 81.75 \\
%				LSTM (framewise) & 47.71 & 70.00\\ 
%				LSTM (segmental)  & 51.25 & 69.80\\ 
%				tCNN (framewise)  & 45.67 & 82.12\\ 
%				tCNN (segmental) & 55.50 & \textbf{82.14} \\ 
%				\hline
				\hline
				\textbf{Holistic Features}  & \textbf{Edit} & \textbf{Accuracy}\\
				\hline				
				IDT   & ? & 56.29 \\ 				
%				sCNN (framewise)  & ? & 56.29 \\ 
				IDT+LSTM   & ? & ? \\
				IDT+Evo   & ? & 61.46 \\
				\hline
				\textbf{Our model}  & \textbf{Edit} & \textbf{Accuracy}\\
				\hline				
				Scene  & 24.10 & 66.64\\ 
				Scene+LSTM  & ? & ?\\
				Scene+Evo  & 49.6 & 69.35\\ 
				Scene+Evo+Seg  &\textbf{55.96} & \textbf{69.36}\\ 
				%CLF  & 65.85 & 69.06\\ 
				\hline
			\end{tabular}
			\end{center}
			\end{minipage}
%			 &
			\begin{minipage}[t]{0.5\linewidth}
			\begin{center}
				\textbf{JIGSAWS} \\
			\begin{tabular}{| l | c | c |}
				%\hline
				%\multicolumn{1}{c}{} & \multicolumn{1}{c}{Framewise} & \multicolumn{1}{c}{Segmental}\\
%				\hline
%				\textbf{Sensor-based}  & \textbf{Edit} & \textbf{Accuracy} \\
%				\hline 
%				\cite{Stefati_m2cai_2015} SD-SDL & -  & 78.68 \\
%				\cite{Lea_icra_2016} LC-SC-CRF & 76.86 & \textbf{83.45}  \\
%				LSTM (framewise)  & 60.94 & 66.32\\ 
%				LSTM (segmental)  & 68.96 & 65.60\\ 
%				%\hline
%				tCNN (framewise)  & 75.78 & 79.00\\ 
%				tCNN (segmental)   & \textbf{82.63} & 79.17\\ 
%				\hline
				\hline
				\textbf{Holistic Features}  & \textbf{Edit} & \textbf{Accuracy}\\
				\hline 			
				IDT			  & ? & 52.70 \\
				IDT+LSTM  & ? & ?\\				 				
				%				sCNN (framewise)  & ? & 56.29 \\ 
				IDT+Evo    & ? & 72.10 \\				
				\cite{tao_miccai_2013} MsM-CRF  & -& 71.78 \\					
				\hline
				\textbf{Our model}  & \textbf{Edit} & \textbf{Accuracy}\\
				\hline
				Scene  & 17.44 & 57.80\\ 
				Scene+LSTM  & ? & ?\\				
				Scene+Evo  & 71.23 & 74.59\\ 
				Scene+Evo+Seg &  \textbf{82.16} & \textbf{74.75}\\ 
				\hline
			\end{tabular}
			\end{center}
			\end{minipage}
%		\end{tabular}
%	\end{center}
	\caption{ Results on 50 Salads and JIGSAWS. }
	\label{table:results1}
\end{table}


%-------------------------------------------------------------
%-------------------------------------------------------------
Table~\ref{table:results2} shows performance on all four action granularities from 50 Salads. All results are computed using the complete spatiotemporal model with segmental inference. The first two scores are using the framewise and segmental metrics. The last score is for the classification regime in which we assume known temporal segmentation. To compute these results we simply take the mean of scores $s_t$ across a given time period and take the best scoring class. 

%1low & 39.88 & 28.56 & 30.97 \\ 
%1mid & 54.11 & 47.79 & 31.27 \\ 
%1eval & 71.4 & 65.49 & 44.47 \\ 
%1high & 91.69 & 74.74 & 37.23 \\
\begin{table}
%\begin{center}
	\begin{minipage}[t]{0.5\linewidth}
			\begin{center}		
%	\begin{tabular}{cc}
		% -----------Hierarchy----------
		\begin{tabular}{| l | c |c | c || c |}
%		\hline
%		\textbf{Sensors} & \textbf{Classes} & \textbf{Edit} & \textbf{Acc.}  & \textbf{Classif.} \\
%		\hline
%		Low & 52  & 30.19 & 50.37 &  26.86\\
%		Mid   & 18 &  36.10 & 58.33 &   44.03\\
%		Eval   & 10 &  55.50 & 82.14 &   64.32\\
%		High  &  4 &  61.60 & 94.48  &  69.03\\
		\hline
		\textbf{Labels} & \textbf{Classes} & \textbf{Edit} & \textbf{Acc.}  & \textbf{Classif.} \\
		\hline
		Low & 52   &  32.83 &  37.90&  35.56\\
		Mid   & 18 &  43.17 & 56.93 &  55.07\\
		Eval  & 10 &  55.96 & 69.36 &   69.06\\
		High & 4 &  62.85 & 91.54 & 87.50\\
		\hline
		\end{tabular}
			\end{center}		
	\end{minipage}
	\begin{minipage}[t]{0.5\linewidth}
					\begin{center}
		\begin{tabular}{| l |  c | c | c |}
			\hline
			\textbf{Labels} & \textbf{Dur} & \textbf{\#Segs} & \textbf{Speedup} \\		
			\hline
			Low &  2289 & 83 & 28x\\ 
			Mid &  3100 & 40 & 85x \\ 
			Eval & 3100 & 37 & 84x \\ 
			High & 11423 & 10 & 1142x\\ 
			\hline
			JIGSAWS & 1107 & 37 & 30x\\ 				
			\hline 			
		\end{tabular}	
		\end{center}			
	\end{minipage}		
%	\end{tabular}		
%\end{center}
\caption{(left) Performance for each granularity in 50 Salads. (right) The speedup of our algorithm compared with Segmental Viterbi. Dur is the longest segment duration in frames. \# Segs is the maximum number of segments in any video.}
\label{table:results2}
\end{table}

%-------------------------------------------------------------
%-------------------------------------------------------------
%The third experiment measures how well the learned representations from the spatial component of our model transfer to different tasks. In each experiment, we train the spatial weights on one granularity from 50 Salads (or JIGSAWS) and test on another. The temporal model is learned on the evaluation granularity. Results are shown in Table~\ref{table:results3}

%\begin{table}
%\begin{center}
%% -----------Hierarchy----------
%\begin{tabular}{| l | c | c | c | c || c |}
%\hline
% & Low & Mid & Eval & High & JIGSAWS\\
%\hline 
%Low & - & - & - & - & -\\ 
%Mid & - & - & - & - & -\\ 
%Eval & -  & - & - & - & -\\ 
%High & - & - & - & - & -\\ 
%\hline
%JIGSAWS & - & - & - & - & -\\ 
%\hline
%\end{tabular}
%\end{center}
%\caption{Experiments 3: Transfer}
%\label{table:results3}
%\end{table}

Lastly, Table~\ref{table:speedup} shows the speedup of our inference algorithm compared to Segmental Viterbi on all 50 Salads and JIGSAWS label sets.


%\begin{table}
%\begin{center}
%% -----------Hierarchy----------
%\begin{tabular}{| l |  c | c | c |}
%\hline
%\textbf{Labels} & \textbf{Duration} & \textbf{\# Segs} & \textbf{Speedup} \\
%\hline 
%Low &  2289 & 83 & 27x\\ 
%Mid &  3100 & 38 & 82x \\ 
%Eval &3100 & 35 & 88x \\ 
%High & 11423 & 6 & 1903x\\ 
%JIGSAWS & 350 & 29 & 12x\\ 
%\hline
%\end{tabular}
%\end{center}
%\caption{The speedup of our algorithm compared with Segmental Viterbi. Max duration is the longest segment duration in frames. Max segments is the maximum number of segments in any video.}
%\label{table:speedup}
%\end{table}

%\THOUGHT{what about combining the sensors and the video in results/experiments?}


==> sections/evaluation_old.tex <==
\section{Evaluation Setup}
\label{sec:evaluation}

In this section we introduce our datasets, metrics, and results on the University of Dundee 50 Salads dataset~\cite{stein_ubicomp_2013} and the JHU-ISI Gesture and Skills Assessment Working Set (JIGSAWS)~\cite{jigsaws-m2cai}. While 50 Salads was developed by researchers in the ubiquitous computing community, we believe it provides great value to the computer vision community due to the large number of action instances per class, the high quality labels, plethora of data, and multi-modal sensors. This dataset can be used to answer many research questions regarding fine-grained action analysis. 

%\TODO{uncomment comparison with other datasets?}
%Many current fine-grained action recognition datasets are limited by size. The MPII Cooking dataset is offers a realistic cooking environment and many different activities, however, many action labels are rarely used. For example, 7 actions (of \TODO{64?} are performed less than 10 times. Similarly, the Georgia Tech Egocentric Activities dataset is nice because if has 7 unique tasks, however, but there are only 3 users to test on and one for evaluation. 


%In this section we discuss the two datasets, our evaluation metrics, and experiments using our models. 

%We perform a comprehensive set of experiments to show ablative analysis, the effect of training on different action granularities,
%and how our model performs if we assume temporal segmentation. Note that our emphasis is not on how the accuracy alone improves, but on how well the segments are modeled. For many applications having a set of cohesive segments is at least, if not more, important than good accuracy. 


%We perform a set of experiments: (1) How does each component of our model (spatial, spatial-temporal, segmental) contribute to overall performance? (2) How does using finer- versus coarser-grained action labels impact performance? (3) Does performance change if we train with a set of finer-grained set of labels than we need? (4) Can we train on one fine-grained dataset and test on another in a different domain? (5) How does our model perform if we have known temporal segmentation? \TODO{say this in words}

%\TODO{reference ICRA paper}

\fakesubsection{University of Dundee 50 Salads}
Stein and McKenna introduced 50 Salads \cite{stein_ubicomp_2013} for evaluating fine-grained action recognition in the cooking domain. This dataset includes 50 instances of salad preparation where each of the 25 users makes a salad in two different trials. Trials include video, depth maps (via Kinect), and synchronized 3-axis accelerometer data from 10 kitchen objects. These accelerometers can be used as a proxy for which objects are being used in the scene. The objects are: \textit{plate}, \textit{pepper dispenser}, \textit{bowl}, \textit{oil bottle}, \textit{large spoon}, \textit{dressing glass}, \textit{knife}, \textit{peeler}, \textit{small spoon}, and \textit{chopping board}.

Videos are annotated at four levels of granularity. The coarsest level (``high'') consists of labels \textit{cut and mix ingredients}, \textit{prepare dressing}, and \textit{serve salad}. At the second tier (``mid'') there are 17 fine-grained actions like \textit{add vinegar}, \textit{cut tomato}, \textit{mix dressing}, \textit{peel cucumber}, \textit{place cheese into bowl}, and \textit{serve salad}. At the finest level (``low'') there are 51 actions indicating the start, middle, and end of the previous 17 actions. For each granularity there is also a \textit{background} class. All actions are listed in the supplemental material. 

%The second granularity (``eval") adds object-agnostic actions like \textit{cutting} 
%%consolidates object-specific actions like \textit{cutting a tomato} and \textit{cutting a cucumber} into a . 
%%For example instead of having a separate action for \textit{cutting a cucumber} and \textit{cutting cheese} there is a single \textit{cutting} action. 
%These actions are: \textit{add dressing, add oil, add pepper, cut, mix dressing, mix ingredients, peel, place} and \textit{serve salad}.

A fourth granularity (``eval"), suggested by \cite{stein_ubicomp_2013}, consolidates some object-specific actions like \textit{cutting a tomato} and \textit{cutting a cucumber} into object-agnostic actions like \textit{cutting}.
%For example instead of having a separate action for \textit{cutting a cucumber} and \textit{cutting cheese} there is a single \textit{cutting} action. 
Actions include \textit{add dressing}, \textit{add oil}, \textit{add pepper}, \textit{cut}, \textit{mix dressing}, \textit{mix ingredients}, \textit{peel}, \textit{place}, \textit{serve salad on plate}, and \textit{background}. These labels coincide with the tools instrumented with accelerometers.

%Our sensor-based results use the same features as \cite{Lea_icra_2016} which are the absolute value of the accelerometer values. We use the same splits with 5-fold validation where we train on 20 users and test on 5 users.

%\subsubsection{50 Salads}
%50 Salads \cite{Stein_2013b} is a multimodal dataset that includes time-synchronized video, depth, and accelerometer data. There are 50 five- to 10-minute samples of a user making a salad. In total there are 25 users -- each of whom makes a salad in two different videos. As shown in figure~ref{fig:salads} a static RGBD camera is mounted facing down looking at the user preparing the salad. Each kitchen utensil has an accelerometer attached that records motion. These can be used to indicate which tools is being used at any given time. In total there are 10 accelerometers. These are located on the following kitchen tools: \textit{plate, pepper\_dispenser, bowl, oil\_bottle, large\_spoon, dressing\_glass, knife, peeler, small\_spoon, chopping\_board}.
%
%One novelty of this dataset is that there are multiple granularities of action labels. At the coarsest there are three actions: \textit{cut\_and\_mix\_ingredients, prepare\_dressing, serve\_salad.} At the most fine-grain it has labels for the start, core, and end of 17 different action primitives such as \textit{add\_vinegar, cut\_tomato, mix\_dressing, peel\_cucumber, place\_cheese\_into\_bowl, serve\_salad.} Following the work of \cite{Stein_2013,Stein_2013b,Yang_Humanoids_2014}, we use the following set of 10 labels for this paper: \textit{add\_dressing, add\_oil, add\_pepper, cut, mix\_dressing, mix\_ingredients, peel, place, serve\_salad\_onto\_plate}. This is a set of hybrid labels that combines types of cutting and placing actions.
%
%In our experiment we only use the accelerometer data. It is reasonable to assume that we could learn object detectors for each of the tools which could be used in place of the accelerometers for purely vision-based applications. 
%
%We evaluate on use the set of 10 action labels from \cite{Stein_2013b}.
%\TODO{ the other relevant papers:} \cite{Stein_2013,Stein_2013b,Yang_Humanoids_2014}

\fakesubsection{JHU-ISI Gesture and Skill Assessment Working Set (JIGSAWS)}
JIGSAWS \cite{jigsaws-m2cai} was developed for recognizing fine-grained actions common in robotic surgery training tasks like suturing, needle passing, and knot tying. This includes about 40 trials of each task including synchronized video and robot kinematics data collected from a daVinci medical robot. The video is taken overhead from an endoscopic camera and depicts two tools and the training task apparatus. 
In our work we just look at the suturing task.
There are eight users and five trials per user. 
The suturing task consists of 10 fine-grained actions such as \textit{insert needle into skin}, \textit{tie a knot}, \textit{transfer needle between tools}, and \textit{drop needle at finish}.
Videos last about two minutes and contain 15 to 37 action instances per video. 

We evaluate using Leave One User Out as suggested by \cite{jigsaws-m2cai} \TODO{change ref}. 
Most prior work on this dataset focuses on the kinematics data such as positions, velocities, and robot joint information. We compare against \cite{tao_miccai_2013} who provide video-only results. Their approach uses holistic features with a Markov Semi-Markov CRF.

%In the sensor-based baseline we use the robot kinematics and vision-based features from the authors of \cite{lea_wacv_2015}. The features are: left and right tool positions, velocities, and gripper angles as well as the distance from the tools to the closest object in the scene from the video.

%------------------------------------------------------------------------------------
\fakesubsection{Metrics}
We evaluate on segmental and frame-wise metrics as suggested by \cite{lea_icra_2016} for the 50 Salads dataset. The first measures segment \textit{cohesion} and the latter captures overall \textit{coverage}. 
%and the other measures overall prediction accuracy. 

In many applications there is high uncertainty in the location of temporal boundaries. Different annotators may have different interpretations of when an action starts or ends. For example, should \textit{cutting} start when a user reaches for the knife or after the knife is in hand? 
%The start or end of an action may be ambiguous or different annotators may interpret an action differently. 
As such, the precise location of temporal boundaries may be inconsequential. In other applications, like human-robot interaction, having cohesive segments is more important. For example, if predictions oscillate between two states in a short amount of time (e.g. $AABABAAA$), despite having a high overall accuracy, the system may not function properly. These over segmentation errors should be penalized.

A segmental edit score, $A_{edit}(G,P)$ allows for slight temporal deviations between the ground truth and predictions but penalizes over segmentation.
This score is computed using the Levenshtein distance which is a function of segment insertions, deletions, and substitutions \cite{?}. Let the ground truth segments be $G=\{G_1,\dots, G_M\}$ and predicted segments be $P=\{P_1,\dots, P_N \}$. The number of edits is normalized by the maximum of $M$ and $N$. For clarity we show the score $(1-A_{edit}(G,P)) \times 100 $ which is a number from 0 to 100. 
% 

%We compute the normalized Levenshtein edit distance $A_{edit}(G',P')$ using the Wagner-Fischer algorithm which penalizes segment insertions, deletions, and substitutions. 

Frame-wise accuracy measures the percent of correct frames in a sequence. 
%and is useful for determining how This is important for coverage. 
%coverage
%Due to issues in inter-annotator variability the score may be sufficient 
Let $G=\{y_1,\dots,y_T\}$ be ground truth labels and $P=\{y^*_1,\dots,y^*_T\}$ be the predicted labels. The score is a function of each frame: $A_{acc}(G,P)=\frac{1}{T} \sum_{t=1}^T \mathbf{1}(G_t=P_t)$. 

We also include action classification results which assume temporal segmentation. These use the accuracy metric applied to segments instead of individual frames. Classification predictions are computed by averaging the scores $s_t$ from the start to end of a given action and taking the best scoring class. 

%measures the overlap between ground truth and predicted segments. It is especially important for applications in human-robot collaboration. 
%This metric is similar to a Jaccard Index but penalizes for gratuitous oversegmentation, such as those resulting from oscillations in action predictions. %This score ranges from 0 to 100 and a higher score is better. 


%The second metric accounts for slight temporal shifts in the prediction. In many domains there is large inter-annotator variability in labeling where temporal boundaries should be located. In applications like surgical skill evaluation the ordering of the actions may matter more than the precise location of the segments. 
%To measure this error we use a segmental edit score. For each ground truth and predicted labeling we first output the sequence of actions (independent of segmentation boundaries). We then compute a normalized edit distance, $s_e(G,P)$, using the Wagner-Fischer algorithm. To make it easier to interpret the results we show scores for $(1-s_e(G,P))*100$. The best score 100 and the worst is 0.

%Note that for convenience in interpreting the results we normalize this score using the length of the ground truth sequence. The best score is 0 and it is unbounded from above. A lower score is better.


%------Metrics when I was planning on using the overlap score----
%%------------------------------------------------------------------------------------
%\subsection{Metrics}
%\THOUGHT{use the segmental edit distance instead. it shows larger discrepancy in segmental model}
%We compute two evaluation metrics: framewise accuracy and a segment-level overlap function. The segmental method was proposed by \cite{ICRA} and measures the overlap between ground truth and predicted segments. It is especially important for applications in human-robot collaboration. 
%This metric is similar to a Jaccard Index but penalizes for gratuitous oversegmentation, such as those resulting from oscillations in action predictions. Given a ground truth sequence $G$ and predicted sequence $P$ the score is:
%\begin{equation}
%A(G, P) = \frac{100}{N} \sum_{i=1}^M \max_j \frac{G_i \cap P_j}{G_i \cup P_j}
%\end{equation}
%This score ranges from 0 to 100 and a higher score is better. 
%
%%The first score measures how much overlap there is between the ground truth segments and the predicted segments. A common metric for this is the Jaccard Index. While this does a good job at measuring coverage, it does not penalize for oversegmentation errors. Predictions from models like the Skip Chain CRF will sometimes add spurious false labels within what should be a long contiguous segment. We penalize these errors by defining an overlap score that is a function of the longest contiguous predicted segment for a given ground truth segment. 
%
%%The second metric accounts for slight temporal shifts in the prediction. In many domains there is large inter-annotator variability in labeling where temporal boundaries should be located. In applications like surgical skill evaluation the ordering of the actions may matter more than the precise location of the segments. To measure this error we use a segmental edit score. For each ground truth and predicted labeling we first output the sequence of actions (independent of segmentation boundaries). We then compute a normalized edit distance, $s_e(G,P)$, using the Wagner-Fischer algorithm. To make it easier to interpret the results we show scores for $(1-s_e(G,P))*100$. The best score 100 and the worst is 0.
%
%%Note that for convenience in interpreting the results we normalize this score using the length of the ground truth sequence. The best score is 0 and it is unbounded from above. A lower score is better.
%
%%Accuracy 
%%Accuracy is the traditional way of measuring accuracy for activity recognition. It is computed as the mean of all correct frames: $m_i(y, y^*) = \frac{1}{N} \sum_{i=1}^N \delta(y_i, y_i^*) $ where $\delta$ is 1 if $y_i$ and $y_i^*$ are the same label and 0 otherwise. 
%
%%We also use accuracy, precision, and recall to compare against prior work. These are defined using $TP$, $FP$, $TN$, and $FN$ for true positives, false positives, true negatives, and false negatives.
%%\begin{align}
%%\text{Accuracy }&= \frac{TP+TN}{TP+FP+FN+TN} \\
%%\text{Precision }&= \frac{TP}{TP+FP}\\
%%\text{Recall }&= \frac{TP}{TP+FN}
%%\end{align}

%------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------
\fakesubsection{Baselines}
We are the first group to evaluate video-based results on the 50 Salads dataset. For proper comparison we provide additional baselines to show our model improves over recent methods. We also apply these to JIGSAWS.

Our Dense Trajectory baseline is comparable to Rohrbach \etal~\cite{rohrbach_ijcv_2015} on the MPII dataset. We extract IDT, create a KMeans dictonary ($k=2000$) on the features, and aggregate the dictionary elements into a local histogram use a sliding window of 30 frames. Similar to \cite{bojanowski_eccv_2014} we found HOG alone performed better than the combined features (HOG+HOF+MBH+Traj). For validation we evaluated the IDT baseline on Georgia Tech Egocentric Activities~\cite{?} and performed comparable to Li \etal~\cite{li_cvpr_2015} \TODO{I can't find this number? just for LC-CRF and SC-CRF}. Note that IDT features alone took 18 hours to compute on 50 Salads compared to 5 hours for our CNN features.
%\TODO{mention our IDT results are comparable to Li on GTEA}

We provide two temporal baselines. The first is a simple sliding SVM comparable to \TODO{which team?} in the THUMOS 2015 action localization challenge and the second uses a Recurrent Neural Net with LSTM. LSTM baseline was implemented in Keras and uses one layer of LSTM units with 64 latent nodes. 

\TODO{put "IDT+Evo" somewhere}


\fakesubsection{Results}
%-------------------------------------------------------------
%-------------------------------------------------------------
Tables~\ref{table:salads} and \ref{table:jigsaws} show performance using the Dense Trajectories (IDT) baseline and our scene model with a sliding SVM, LSTM, and our model. 
We include ablative results for each component of our approach where Scene, Evo, and Seg refer to the models for \textit{scene state}, \textit{intra-action evolution}, and \textit{inter-action transitions}. These 50 Salads results are on the ``eval" granularity. Some example predictions are visualized in Figure~\ref{fig:timeline}.
 
Table~\ref{table:granularities} shows performance on all four action granularities from 50 Salads using our full model. The first two scores show scores for segmental and frame-wise metrics. The last score is for action classification in which we assume known temporal segmentation. Table~\ref{table:speedup} shows the speedup of our inference algorithm compared to Segmental Viterbi on all 50 Salads and JIGSAWS label sets.

On 50 Salads Lea \etal~\cite{lea_icra_2016} showed results using the instrumented kitchen tools. They achieved an edit score of 58.46\% and accuracy of 81.75\%.
They also achieve state of the art performance on JIGSAWS with 78.91\% edit and 83.45\% accuracy.
Note we do not expect to achieve as high performance from video. These results used domain-specific sensors which are well suited to each application but may not be practical for real-world deployment. To contrast, video is much more practical for deployment but is more complicated to model. 
 
%We provide a matrix of experiments showing the effect of each spatial and temporal model. We evaluate using two spatial features: our CNN and a Dense Trajectory baseline. Furthermore, we use each set of spatial features as input into the temporal models. We have three temporal models: a Sliding SVM baseline, an RNN-LSTM baseline, our intra-action model, and our full model. 

%The Sliding SVM is comparable to Rohrbach \etal~\cite{rohrbach_ijcv_2015} where we use a sliding window of 30 frames.

%we achieve 56.29\% accuracy on the 50 Salads ``eval'' set and 52.70\% on JIGSAWS.  
%We also experimented using the IDT-based frame-level features as input into our temporal CNN. We achieve 61.46\% and 72.10\% respectively on these datasets. 
%All IDT results are lower than from the full model in our paper.
%These results are consistent with findings of Li \etal (CVPR15) on the Georgia Tech Egocentric Activities dataset and in the CVPR2015 THUMOS action localization challenge. 
%While IDT are great for large-scale action classification, we found they do not capture nuances of fine-grained action segmentation and classification. 



%-------------------------------------------------------------
%-------------------------------------------------------------



%1low & 39.88 & 28.56 & 30.97 \\ 
%1mid & 54.11 & 47.79 & 31.27 \\ 
%1eval & 71.4 & 65.49 & 44.47 \\ 
%1high & 91.69 & 74.74 & 37.23 \\
\setcounter{table}{0}
\begin{table}
%\begin{center}
			\begin{minipage}[t]{0.5\linewidth}
				\begin{center}
%					\textbf{50 Salads} \\
					\begin{tabular}{| l | c | c |}
						\hline
						\textbf{Holistic Features}  & \textbf{Edit} & \textbf{Accuracy}\\
						\hline				
						IDT   & 7.76 & 56.35 \\ 				
						IDT+LSTM   & ? & ? \\
						IDT+Evo   & ? & 61.46 \\
						\hline
						\textbf{Our model}  & \textbf{Edit} & \textbf{Accuracy}\\
						\hline				
						Scene  & 24.10 & 66.64\\ 
						Scene+LSTM  & 58.84 & 66.30 \\ 
						% clf = 74.63
%						Scene+LSTM+Seg  & 61.43 & 66.33 \\						
						Scene+Evo  & 60.98 & 71.37 \\ 
						Scene+Evo+Seg  &\textbf{62.06} & \textbf{72.00}\\ 
%						ICRA: Scene+Evo  & 62.63 & 72.21\\ 
%						ICRA: Scene+Evo+Seg  &\textbf{66.44} & \textbf{72.71}\\ 
%						(no prior) SE  & 60.68 & 69.75\\ 						
%						(no prior) SES  & 63.02 & 69.58\\
						\hline
					\end{tabular}
				\caption{50 Salads}					
				\label{table:salads}
				\end{center}
			\end{minipage}
			%			 &
			\begin{minipage}[t]{0.5\linewidth}
				\begin{center}
%					\textbf{JIGSAWS} \\
					\begin{tabular}{| l | c | c |}
						\hline
						\textbf{Holistic Features}  & \textbf{Edit} & \textbf{Accuracy}\\
						\hline 			
						IDT			  & 8.45 & 53.92 \\
						IDT+LSTM  & ? & ?\\				 				
						%				sCNN (framewise)  & ? & 56.29 \\ 
						IDT+Evo    & ? & 72.10 \\				
						\cite{tao_miccai_2013} STIPS+CRF  & -& 71.78 \\					
						\hline
						\textbf{Our model}  & \textbf{Edit} & \textbf{Accuracy}\\
						\hline
						Scene  & 20.10 & 67.25\\ 
						Scene+LSTM  & 54.07 & 68.37\\				
%						Scene+LSTM+Seg  & 58.71 & 68.77\\
						Scene+Evo &  59.89 & 71.21\\
						Scene+Evo+Seg &  \textbf{66.56} & \textbf{74.22}\\
						% clf=90.47
%						ICRA: Scene+Evo &  54.96 & 74.80\\
%						ICRA: Scene+Evo+Seg &  \textbf{70.74} & \textbf{74.89}\\
						% clf = acc=92.56, edit=92.62
%						(no prior) SE  & 71.23 & 74.59\\ 						
%						(no prior) SES &  82.16 & 74.75\\
						\hline
					\end{tabular}
				\end{center}
				\caption{JIGSAWS}
				\label{table:jigsaws}
			\end{minipage}
			\\
			\\
			\\
	\begin{minipage}[t]{0.5\linewidth}
			\begin{center}		
%			\textbf{50 Salads Granularities}\\				
%	\begin{tabular}{cc}
		% -----------Hierarchy----------
		\begin{tabular}{| l | c |c | c || c |}
%		\hline
%		\textbf{Sensors} & \textbf{Classes} & \textbf{Edit} & \textbf{Acc.}  & \textbf{Classif.} \\
%		\hline
%		Low & 52  & 30.19 & 50.37 &  26.86\\
%		Mid   & 18 &  36.10 & 58.33 &   44.03\\
%		Eval   & 10 &  55.50 & 82.14 &   64.32\\
%		High  &  4 &  61.60 & 94.48  &  69.03\\
		\hline
		\textbf{Labels} & \textbf{Classes} & \textbf{Edit} & \textbf{Acc.}  & \textbf{Classif.} \\
		\hline
		% =====ICRA results=====	
		\hline
		icra (saturday)  & & & & \\
		Low & 52   & 29.30  & 44.13 & 39.67 \\
		Mid   & 18 &  48.94 & 58.06  & 63.49 \\
		Eval  & 10 & 66.44  & 72.71 &  86.63\\
		High & 4 & 83.2  & 92.43 & 95.14 \\		
%		\hline
%		icra (saturday)  & & & & \\
%		Low & 52   & 29.30  & 44.13 & 39.67 \\
%		Mid   & 18 &  48.94 & 58.06  & 63.49 \\
%		Eval  & 10 & 66.44  & 72.71 &  86.63\\
%		High & 4 & 83.2  & 92.43 & 95.14 \\
		\hline
		old & & & & \\
		% =====Results from CVPR=====		
		Low & 52   &  32.83 &  37.90&  35.56\\
		Mid   & 18 &  43.17 & 56.93 &  55.07\\
		Eval  & 10 &  55.96 & 69.36 &   69.06\\
		High & 4 &  62.85 & 91.54 & 87.50\\
		\hline
		\end{tabular}
		\caption{50 Salads Granularity Analysis}
		\label{table:granularities}
		\end{center}		
	\end{minipage}
	\begin{minipage}[t]{0.5\linewidth}
		\begin{center}
%		\textbf{Speedup Analysis}\\
		\begin{tabular}{| l |  c | c | c |}
			\hline
			\textbf{Labels} & \textbf{Dur} & \textbf{\#Segs} & \textbf{Speedup} \\		
			\hline
			Low &  2289 & 83 & 28x\\ 
			Mid &  3100 & 40 & 85x \\ 
			Eval & 3100 & 37 & 84x \\ 
			High & 11423 & 10 & 1142x\\ 
			\hline
			JIGSAWS & 1107 & 37 & 30x\\ 				
			\hline 			
		\end{tabular}
		\caption{Speedup Analysis}
		\label{table:speedup}
		\end{center}			
	\end{minipage}		
%	\end{tabular}		
%\end{center}
%\caption{(left) Performance for each granularity in 50 Salads. (right) The speedup of our algorithm compared with Segmental Viterbi. Dur is the longest segment duration in frames. \# Segs is the maximum number of segments in any video.}
%\label{table:results2}
\end{table}

%-------------------------------------------------------------
%-------------------------------------------------------------
%The third experiment measures how well the learned representations from the spatial component of our model transfer to different tasks. In each experiment, we train the spatial weights on one granularity from 50 Salads (or JIGSAWS) and test on another. The temporal model is learned on the evaluation granularity. Results are shown in Table~\ref{table:results3}



==> sections/framewise_models.tex <==
\section{Framewise Models}
\label{sec:framewise}

First we introduce the generic framework for our Framewise Model (FM). Then we describe learning and inference. Finally, we define our potentials. An instantiation of one of our models is depicted in figure~\ref{fig:models}. 

\subsubsection{Model}
Let the variable $X_t$ be a set of features at time $t$ for $1\leq t \leq T$ and $Y_t$ be the corresponding action. Given a sequence of data $X$ and labels $Y$ we define an energy function $E(X,Y)$ as a linear function of weight vectors $w_i$ and potentials $\phi_i(X,Y)$ for $i=\{1...P\}$. 
\footnote{For clarity we choose to define weights and potentials as vectors. In practice, it is common to represent the weights as matrices where elements are indexed based on the labels (e.g. compute the unary $w_a^T X_t$ for $Y_t=a$ and $w_b^T X_{t+1}$ for $Y_{t+1}=b$ where $w_a$ and $w_b$ are the weight vectors for classes $a$ and $b$). This notation is common practice and is without loss of generality.}
These potentials may model various components like the data at time $t$, the transition between actions or features from time $t-d$ to $t$, or a prior on what action is likely at $t$.
Our energy is given by:
\begin{align}
	E(X,Y) = \sum_{t=1}^T \sum_{i=1}^P w_i^T \phi_i(X, Y)
\end{align}

%\begin{align}
%\left[
%\begin{array}{l}
%\sum_{i=1}^M \text{w}_{s}^T \phi (X, y_i, s_{i}, e_{i}) + \\
%\sum_{i=2}^M \text{w}_{p}^T \psi (y_i, y_{i-1})
%\end{array} 
%\right] 
%\end{align}

Note that in a probabilistic setting this model can be viewed as a Linear Chain Conditional Random Field using the the Gibbs distribution $P(Y | X) = \frac{1}{Z} \exp(-E(X, Y))$ with partition function $Z$.

Next we define a loss function $\Delta(Y^*, Y)$ given the ground truth labeling $Y^*$ and any arbitrary labeling $Y$. This loss is used to compute the empirical risk and should be similar with how we measure accuracy in Section~\ref{sec:evaluation}. For all framewise models we use the Hamming loss: 

\begin{align}
\Delta(Y^*, Y) = \sum_{t=1}^T \mathbf{1}[Y^*_t \neq Y_t]
\end{align}
 
\subsubsection{Learning}
There are many objectives for which we could learn the weights for our model. These include probabilistic maximum likelihood models (c.f. Conditional Random Fields), mean-squared error (c.f. Recurrent Neural Networks), or Max-Margin models (c.f. Max Margin Markov Nets \cite{taskar_nips_2003}). Recent work has shown that the Structural Support Vector Machine (SSVM) objective achieves superior performance than its competitors and can be computed more efficiently \cite{?,PAMI-ProbVsDisc,Muller2013}. Thus, we jointly learn all weights $w=[w_1,...,w_P]$ using the Structural Support Vector Machine \cite{tsochantaridis_jmlr_2005}. This objective models the upper bound on the empirical risk of our data using the aforementioned loss function $\Delta$.

Let a sample sequence of data be $X^{(n)}$ and its corresponding labels be $Y^{(n)}$. Let $\Psi(X,Y)=\sum_{i=1}^T V(t, Y_t^{(n)} )$ be the joint feature function. The objective function is given by:
%
\begin{align}\label{eq:learning}
\min_{w, \xi} || w ||^2 + & C \sum_{n=1}^{N} \max_Y \Delta(Y_*^{(n)}, Y) \nonumber \\
+ & w^T(\Psi(X^{(n)}, Y) - \Psi(X^{(n)}, Y_*^{(n)})) 
\end{align}

\TODO{talk about loss augmented inference}

We minimize Equation~\eqref{eq:learning} using Stochastic Gradient Descent. The step sized is computed dynamically with Adagrad~\cite{Duchi_2010}. We find this is faster and provides superior performance over other recent methods such as Block Coordinate Frank Wolfe~\cite{lacoste-julien_icml_2013}. We have implemented all of these models and learning algorithms in Struct.jl, our structured prediction library \footnote{\url{https://github.com/colincsl/struct.jl}}. For more details on this model see \cite{Nowozin2010}.
  

\begin{figure*}
\center
	\includegraphics[width=.3\hsize]{imgs/models/LM}
	\includegraphics[width=.3\hsize]{imgs/models/HLM}
	\includegraphics[width=.3\hsize]{imgs/models/SM}
	\caption{Hierarchical Semi-Markov Conditional Random Field }
	\label{fig:models}
\end{figure*}

\subsubsection{Inference}
We infer the best possible labeling $Y=\arg\max_Y E(X,Y)$ by maximizing the cost of all potentials $phi_i$ at each frame. During inference, we maintain a score $V(t, y)$ for each label $y$ at all timesteps $t$ where $V(t,y) = \sum_i=1^P w_p^T \phi_i(X, y)$. Potentials can been added in an arbitrary order, however, for improved accuracy any potential that pools over the class at another timestep (e.g. a pairwise class transition term) should be applied at the end.
\footnote{Note, when just using the following data and pairwise-class potentials we could perform inference using the Viterbi algorithm \cite{Rabiner1989}. The update score for our pairwise-class term effectively does this. However, in practice we find that independently summing over an arbitrary set of potentials makes it easier to develop more interesting and complex models.}

The computational complexity of inference varies depending on the potentials used. Inference for the baseline case where we only have potentials on data and pairwise class transitions has complexity of $O(TC)$ and $O(TC^2)$ respectively where $C$ is the number of classes. 

%\begin{tabular}{c c}
%\hline
%variable & description
%\hline
%$X$
%\hline
%\caption{Table of variable names}
%\end{tabular}

% --------------------------------------------------------------------------------------
\subsection{Potentials}
Here we define a unary data potential, pairwise class- and feature-transition potentials, temporal priors, and hierarchical potentials.

\subsubsection{Data Potential}
First we want to learn a weight for each feature and class based on the data at a given timestep. Note that $X_t$ here could be raw data (e.g. pixels or robot kinematics) or the output of another classifier (e.g.  activations from a Convolutional Neural Net). Thus, the cost of the data over a sequence for a label $y=c$ is simply the sum of the data for all timesteps where $y^*=c$. 

\begin{align}
C_{d}(X, y=c) = \sum_{t=1}^T X_t \cdot \mathbf{1}[y_t=c]
\end{align}

If this is the only term in our model and we use the Hamming loss function then this is the special case of a multi-class Support Vector Machine.

% ----------------------------------------------------------------------------
\subsubsection{Pairwise Class Skip-frame Potential}
Our second term is a generalization of the common pairwise class potential used in linear chain Markov models which we first presented in \cite{lea_wacv_2015}. This term models the cost of transitioning into class $b$ at time $t$ from class $a$ at time $t-d$ where $d$ is our skip-length. The motivation is as follows. The typical Markov assumption assumes a class transition from time $t-1$ to $t$ ($d=1$). Video and other sensor data typically has a framerate of 30 frames per second. Thus, the Markov assumption tends to want to stay in the same class from frame-to-frame; there is a high probability that $y_{t-1}=y_t$. If our skip length is similar to the length of an average action then we will tend to transition into a different action every $d$ frames; there is a high probability that $y_{t-1} \neq y_t$. In practice we see the pairwise transition matrices look very different for various values of $d$.

This cost is modeled as:
\begin{align}
C_{pc}(X, y) = \sum_{t=2}^T \mathbf{1}[y_{t-d}=c_1,y_t=c_2]
\end{align}

\TODO{show inference (using pooling) for this term}

\subsubsection{Pairwise Data Transition Potential}
Next we look at how the features change as we change between different classes. Define $f(X_{t-d}, X_t)$ to be a function of the features from the previous timestep to the current timestep. We define this as the difference function $f(X_t, X_{t-d}) = X_t - X_{t-d}$. Another example function is the Euclidian distance between features. The motivation behind using this term is that it can help determine when an action has transitioned from one class to another. Assuming the features are similar within a class then the cost should be low within classes and high outside of a class.

This cost is modeled as:
\begin{align}
C_{pd}(X, y) = \sum_{t=2}^T f(X_t, X_{t-d}) \cdot \mathbf{1}[y_{t-d}=c_1,y_t=c_2]
\end{align}

% ----------------------------------------------------------------------------
\subsubsection{Class Prior}
The next few potentials are priors that model how likely a class is to appear at any given time. The first prior is the most general and models the cost of seeing a particular label regardless of time. This is equivalent to a bias term in an affine model. Intuitively we want to positively bias classes we see frequently and negatively bias classes we see infrequently.

This cost is modeled as:
\begin{align}
C_{c}(y) = \sum_{t=1}^T \mathbf{1}[y_t=c]
\end{align}

\subsubsection{Boundary Priors}
Typically in fine-grained applications there are many different sequences that all constitute the same activity. For example, if you are making a peanut butter and jelly sandwich you can spread peanut butter on bread before jelly or after. However, typically in these settings there are only one or two ways to start and end a sequence. For example, you must start the sandwich making activity by picking up the bread. 

Second, we focus on the start and the end of a sequence. We add an addition bias for what action class we should see at the beginning of the sequence and a separate bias for the end of the sequence. These are modeled as follows assuming $d$ is the average length of a segment:

Start:
\begin{align}
C_{bs}(y) = \sum_{t=1}^d \mathbf{1}[y_t=c]
\end{align}


End:
\begin{align}
C_{be}(y) = \sum_{t=T-d}^T \mathbf{1}[y_t=c]
\end{align}

\subsubsection{Temporal Priors}
For the last prior we model the cost of seeing an action at any specific time $t$ within a sequence. We see that in some applications there are some actions that always occur earlier in the sequence and others that occur later in the sequence. There is one issue: our sequences all have a different number of timesteps. Thus, for this cost we scale all sequences to a canonical sequence length $T'$. In practice, we set $T'$ to be much smaller than the total number of frames (e.g. $T'=50$ for sequences around $T \approx 2000$.). This helps with smoothing and reduces the number of parameters which helps with overfitting.

To transform the data into the canonical sequence length let $t'=t \frac{T}{T'}$. Our cost is then modeled as:
\begin{align}
C_{t}(X, y, t) =  \mathbf{1}[y_{t'}=c] 
\end{align}


% ----------------------------------------------------------------------------
\subsubsection{Deep Model}
For clarity we make a small change to our energy function for the hierarchical potentials. We introduce a new variable, $l$ which is the current layer in the hierarchy where $1 \leq l \leq L$. In addition, the labels, denoted $Y^l$, are the set of most likely labels for some layer in the hierarchy. For example, if the bottom layer has labels $Y=Y^1=[AABBBB]$ then the second layer may be $Y^2=[ABB]$. The updated energy is:

\begin{align}
	E(X,Y) = \sum_{l=1}^L \sum_{t'=1}^{T'} \sum_{i=1}^P w_i^T \phi_i(X, Y^l)
\end{align}

Any of the previous potentials can now be applied to each of the layers $l$. For example, the hierarchical data term becomes: 
\begin{align}
C_{hd}(X, y) = \sum_{l=1}^L \sum_{t=1}^T X^{(l)}_t \cdot \mathbf{1}[y_t=c]
\end{align}



==> sections/inference_old.tex <==
\section{Segmental Model of Inter-action Transitions}
\label{sec:inference}
In this section we define our segmental model and introduce an efficient algorithm for performing inference. Later we show that this model improves performance by reducing the number of false-positive action predictions. 
%Note that this is in contrast to most models, including many CNNs, RNNs, and CRFs, which predict the label individually for each frame: $y_t = \argmax\limits_{y} s_t^y$. 

\subsection{Segmental Model}
We encode action-to-action transitions and temporal priors using the Semi-Markov CRF formulation originally proposed by Sarawagi and Cohen~\cite{sarawagi_nips_2004}. 
This model is used to jointly segments and classify all actions in a sequence.

%We infer the labels for all frames jointly with an inference model first that captures actions at a segment-level. 
%One important advantage of this model is our ability to explicitly capture action-to-action transitions and priors temporal probabilities. 
%We build upon prior work on Semi-Markov CRFs~\cite{sarawagi_nips_2004},shi_ijcv_2011,hu_icra_2014} and Segmental Regular Grammars~\cite{pirsiavash_cvpr_2014}. 

%%In the typical CNN or RNN, the class prediction $y_t$ for each frame is independent of all other frames given the score $s_t$.
%Most CNN and RNN formulations predict a class at each frame independently of all other frames given the current score: 
%$y_t = \argmax\limits_{y} s_t^y$. 
%Thus if the classifier is not confident of the class, meaning scores for classes $a$ and $b$ are similar, then it common for the labels to oscillate from $y_t=a$ to $y_{t+1}=b$ to $y_{t+2}=a$ over a long contiguous sequence. 
%For most applications we prefer a set of coherent segments that do not oscillate between labels over short periods of time. 
%In practice we see these oscillations even occur with models like Long Short Term Memory (LSTM) which capture long-term class state. 

Let tuple $P_j=(y_j, t_j, d_j)$ be the $j$th action segment where $y_j$ is the action label, $t_j$ is the start time, and $d_j$ is the segment duration. There is a sequence of $M$ segments $P=\{P_1,...,P_M\}$ for $0 < M \leq T$ such that the start of segment $j$ coincides with the end of the previous segment $t_j=t_{j-1}+d_{j-1}$ and the durations  sum to the total time $\sum_{i=1}^M d_i = T$.
Given scores $S=\{s_1, \dots, s_T\}$ from Section~\ref{sec:model} we infer segments $P$ that maximize the cost $E(S,P)$ for the whole video using segment function $f(\cdot)$:
\begin{align}
	E(S,P)=\sum_{j=1}^M f(S, y_j, t_j, d_j)
\end{align}
We impose the constraint $y_i \neq y_{i-1}$ for all segments $i$ to avoid the degenerate solution where each consecutive segment receives the same label (e.g. $y_1=y_2=...=a$). We choose $f$ to be the sum function with a constraint on self-transitions:
ointly
\begin{align}
	f(S, y_j, t_j, d_j) = 
\begin{cases}
\sum_{t=t_j}^{t_j+d_j-1} S^{y_j}_t  ,& \text{if } y_j \neq y_{j-1}\\
    -\infty,              & \text{otherwise}
\end{cases}	
\end{align}

\begin{align}
f(S, y_j, t_j, d_j) = 
\begin{cases}
P^j_{y_j} + T_{y_{j-1},y_j} + \frac{1}{d_j} \sum_{t=t_j}^{t_j+d_j-1} S^{y_j}_t  ,& \text{if } y_j \neq y_{j-1}\\
-\infty,              & \text{otherwise}
\end{cases}	
\end{align}
Where $T_{y_{j-1},y_j}$ is the log transition probabilities going from class $y_{j-1}$ to $y_j$ and $P^j_{y_j}$ is a the log prior probability of segment $j$ belonging to class $y_j$. These parameters are learned by computing the corresponding probability distributions from the the training data.



\subsection{Segmental Inference}
Sarawagi and Cohen \cite{sarawagi_nips_2004} introduced this model in the context of a Semi-Markov Conditional Random Field and solve the following discrete constrained optimization problem:
\begin{align}
P^* = \argmax\limits_{P_1,\dots, P_M} \text{ } E(S, P) \quad  s.t. \textstyle \sum_{i=1}^M d_i = T \qquad \mbox{and} \quad  0 < M \leq T 
\end{align}
They introduce an algorithm, which we refer to as Segmental Viterbi, that extends the traditional Viterbi method to the case of joint segmentation and classification. 
The forward pass of their method is shown in Algorithm~\ref{alg:inference} (left) and the optimal labels are recovered by backtracking through the matrix. Let $V$ be a score table of size $T \times C$ which stores the best cost for each time and class.
Conceptually, their approach is frame-wise. For each frame, they compute scores for all possible segment durations, current labels, and previous labels. 
%Their recursive update step is defined as follows with score $V_{y,t}$ for class $y$, time $t$, previous class $y'$ and segment duration $d$: 
%$V_{y,t}=\argmax\limits_{d, y'} V_{y',t-d} + f(S, y, t, d)$. 
In the naive case this results in an algorithm of complexity $O(T^2C^2)$ because the segments can be of arbitrary length. The complexity can be reduced to $O(TDC^2)$ by simply limiting the maximum segment duration, $D$, to an upper bound on the segment lengths.

%is typically maximized over values from $1$ to the maximum segment length $D$. 
%In the forward pass the scores are computed for all timesteps, classes, previous classes, and durations. 
% The computational complexity of this approach is $O(TC^2D)$.

% in addition to optimizing over the they optimizes over all possible durations of each segment. They perform dynamic programming with score table $V$ using the recursive update 
%$V_{c,t}=\argmax\limits_{\substack{d=1...D \\ y'}} V_{y',t-d} + f(X, c, t, d)$
%$V_{c,t}=\argmax\limits_{d, y'} V_{y',t-d} + f(s, c, t, d)$
% In the forward pass the scores are computed for all timesteps, classes, previous classes, and durations. The optimal labels are recovered by backtracing through the matrix. 

We introduce a new algorithm that reduces complexity substantially by computing the scores segment-wise instead of frame-wise. 
We bound the maximum number of action segments to $K$ and solve a slightly modified optimization problem:
%By bounding the maximum number of segments in a video we dramatically decrease the number of necessary computations. 
%\begin{align}
%Y = \argmax\limits_{P_1,\dots, P_M} \text{ } E(S, P) \quad
%s.t. \textstyle \sum_{i=1}^M d_i = T \quad \mbox{and}  \quad   0 < M \leq K \nonumber
%\end{align}
\begin{align}
P^* = \argmax\limits_{P_1,\dots, P_M} \text{ } E(S, P) \quad
s.t. \textstyle   \quad   0 < M \leq K 
\end{align}
Note that we no longer need to optimize over durations because we assume that each timestep is part of one of the segments.
The forward pass of our method is shown in Algorithm~\ref{alg:inference} (right) and the optimal labels are recovered by backtracking. 
Let $V$ be a score table of size $K \times T \times C$ which stores the best cost for each time and class.
Now, for each segment, we maximize over the starting time, current labels, and previous labels. 
If $K$ is the upper bound on the number of segments then our complexity is $O(KTC^2)$.

%Our solution is a different dynamic programming approach in which we compute a score $V'_{k,y,t}$ for all segments $k$, such that $0 < k \leq K$, with recursive update
%\begin{align}
%	V_{k,c,t}=\argmax\limits_{y'} V_{k-1,y',t-d} + f(s, y, t, d)
%\end{align}
%At a high level our approach computes the best labeling for each segment up to $K$ while Segmental Viterbi computes the best labeling for each frame up to time $T$. 
%Our algorithm is detailed in Algorithm~\ref{alg:segmental}. 

%We compute score $V'_{k,c,t}$ where $k$ is the $i$th segment in a sequence. We bound the number of possible segments by $K$ which, for our applications, ranges from 4 to 72. Our algorithm is a straightforward use of Dynamic Programming and is detailed in Algorithm~\ref{alg:segmental}.

%$V_{c,t}=\argmax\limits_{\substack{d=1...D \\ y'}} V_{y',t-d} + f(X, c, t, d)$

\begin{table}%
	\begin{tabular}{cc}
		\begin{tabular}{|c|}
		\hline
		\hspace{0pt}\\		
		\begin{subalgorithm}{.49\textwidth}
			\begin{algorithmic}[b]
				\For{$t=1:T$} 
				\For{$c=1:C$} 
				\State $v_{cur} = V_{t-1,c} + s^{c}_t$ 
				%		\Comment{Keep state} 
				\State $v_{prev} = \max\limits_{\substack{{\color{red}d \in \{1 \dots D\} }\\ c' \in \mathcal{Y}/c }} V_{t-d,c'} + s^{c}_t$  %\Comment{Change state}
				\State $V_{t,c} = \max(v_{cur}, v_{prev})$ %\Comment{Update cost}
				%		\State \hspace{0pt}
				%		\State \hspace{0pt}
				\EndFor
				\EndFor
			\end{algorithmic}
		\end{subalgorithm}\\		
		\hspace{0pt}\\
		\hline
		\end{tabular}
		& 
		\begin{tabular}{|c|}		
		\hline
		\hspace{0pt}\\
		\begin{subalgorithm}{.49\textwidth}
			\begin{algorithmic}[b]
				\For{$k=1:K$ } %\Comment{Segments}
				\For{$t=1:T$ } %\Comment{Time steps}
				\For{$c=1:C$ } %\Comment{Time steps}		
				\State $v_{cur} = V_{k,t-1,c} + s^{c}_t$
				\State $v_{prev} = \max\limits_{c'} V_{k-1,t-1,c'} + s^{c}_t$
				\State $V_{k,t,c} = \max(v_{cur}, v_{prev})$ %\Comment{Update cost}
				\EndFor
				\EndFor
				\EndFor
			\end{algorithmic}
			%			\caption{Our Approach}{}
			%		\label{alg:SegViterbi}
		\end{subalgorithm} \\		
		\hspace{0pt}\\
		\hline
		\end{tabular}\\
		Segmental Viterbi & Our Algorithm
%			\caption{Segmental Viterbi [Cohen]}{} \label{alg:Ours}
	\end{tabular}
	\captionsetup{labelformat=alglabel}
	\caption{The forward pass of our segmental inference algorithm compared with Segmental Viterbi \cite{sarawagi_nips_2004}}%
	\label{alg:inference}%
\end{table}

%\algsetup{linenosize=\small}
%\begin{table}%
%	\fbox{
%%		\vspace{0pt}
%	\begin{minipage}[t][3.5cm]{.48\textwidth}
%	\begin{subalgorithm}{\textwidth}
%		\begin{algorithmic}[b]
%\For{$k=1:K$ } %\Comment{Segments}
%	\For{$t=1:T$ } %\Comment{Time steps}
%		\For{$c=1:C$ } %\Comment{Time steps}		
%			\State $v_{cur} = V_{k,t-1,c} + s^{c}_t$
%			\State $v_{prev} = \max\limits_{c'} V_{k-1,t-1,c'} + s^{c}_t$
%			\State $V_{k,t,c} = \max(v_{cur}, v_{prev})$ %\Comment{Update cost}
%		\EndFor
%	\EndFor
%\EndFor
%		\end{algorithmic}
%		\caption{Our Approach}{}
%%		\label{alg:SegViterbi}
%	\end{subalgorithm}
%	\end{minipage}
%	}
%	\fbox{
%%		\vspace{0pt}
%	\begin{minipage}[t][3.5cm]{.48\textwidth}
%	\begin{subalgorithm}{\textwidth}
%		\begin{algorithmic}[b]
%		\For{$t=1:T$} 
%		\For{$c=1:C$} 
%		\State $v_{c} = V_{t-1,c} + s^{c}_t$ 
%%		\Comment{Keep state} 
%		\State $v_{p} = \max\limits_{\substack{{\color{red}d \in \{1 \dots D\} }\\ c' \in \mathcal{Y}/c }} V_{t-d,c'} + s^{c}_t$  %\Comment{Change state}
%		\State $V_{t,c} = \max(v_c, v_p)$ %\Comment{Update cost}
%%		\State \hspace{0pt}
%%		\State \hspace{0pt}
%		\EndFor
%		\EndFor
%		\end{algorithmic}
%		\caption{Segmental Viterbi [Cohen]}{} \label{alg:Ours}
%	\end{subalgorithm}
%	\end{minipage}
%	} 
%	\captionsetup{labelformat=alglabel}
%	\caption{Forward pass of (left) our segmental inference algorithm and (right) Segmental Viterbi [Cohen]}%
%%	\label{tab:1}%
%\end{table}

%Go through $k$-th segment
%Evaluate at each timestep
% Go through all classes

%Our method has computational complexity of $O(TC^2K)$. 
%The number of segments is much less than the number of frames. 
Assuming $K < D$ our solution is $\frac{D}{K}$ times more efficient than Segmental Viterbi. 
Clearly it becomes more efficient as the ratio of the number of segments $K$ to the maximum segment duration $D$ decreases. 
In most practical applications $K$ is much smaller than $D$. For the datasets in this paper our method results in a speedup of 28x to 1900x on 50 Salads and 30x on JIGSAWS.
One drawback of our solution is its has larger space complexity. Our method is $O(KTC)$ while Segmental Viterbi is $O(TC)$. In practice the increase in memory is manageable on any modern system. 


%Our approach has similar restrictions to Cohen which are implicit in Dynamic Programming problems. Function $f(s, y, t, d)$ must be nonnegative and may not decrease as a segment increases in duration.


%Note that P?? and Ramanan~\cite{ramanan} introduced an algorithm for Segmental Regular Grammars that is very similar to S and Cohen.

%Our algorithm has a computational cost of $(TC^2D)$ where $D$ is the maximum length of a segment. In practice this can be very slow because of the last term which may be on the order of hundreds or thousands of frames. 

%\TODO{Restrictions on this model: $s_t$ is non-negative (implies segment score is non-decreasing)}

%Our algorithm is a special case of Dynamic Programming.

%In this section we develop efficient inference methods for the case where we have a task model for each sequence. We discuss three regimes: the first is the traditional method, the second assumes we have a task model for each sequence, and the third assumes we know the number of actions that occur in a sequence. Lastly we describe how to efficiently perform inference in an online setting.

%\subsection{Viterbi Decoding}
%We infer the best possible labeling $Y=\argmax_Y E(X,Y)$ by maximizing the cost of all potentials $\Psi$ at each frame \cite{rabiner_1989}. During inference, we compute a score $V_{t, y}$ for each label $y$ at all timesteps $t$. $V$ is a table of size $T \times C$ where $T$ is the total time and $C$ is the number of classes. This is a dynamic programming problem where 
%$V_{t,y} = \max_{y'} V_{t-1,y} + w^T \Psi(X, y, y', t)$. 
%We output the best labeling $Y$ by backtracking through the table of scores to find the best scoring sequence. 
%
%\begin{equation}
%	Y = \argmax_{y_i, d_i \forall 0 < i < T} E(X, Y)
%\end{equation}
%\begin{equation}
%	Y = \argmax_{y_i, d_i \forall 0 < i < M} E(X, Y)
%\end{equation}

%	V_{t,y} = \max_{y'} V_{t-1,y} + w^T \Psi(X, y, y', t)


%\subsection{Task Model Decoding}
%In the second regime we assume we have a task model for the particular sequence. This is the special case where we know the order of the actions (e.g. $A \rightarrow B \rightarrow C$) but not when the actions happen temporally. Let the sequence of labels be $S=[c_1, c_2, ..., c_K]$ for actions $c_i$ where $K$ is the total number of segments. This problem becomes $Y=\argmax_Y E(X,Y) \text{ s.t. } S=[c_1, c_2, ..., c_K]$. We can compute the best scores using dynamic programming where $V_{t,k} = \max(V_{t-1,k}, V_{t-1,k-1}) +  w^T \Psi(X, y, y', t)$. The best labeling is computed by backtracing through the table from score $V_{T,|S|}$ to $V_{1,1}$ where $|S|$ is the number of action segments. See Algorithm~\ref{alg:Inference} for how to compute this table.

%\subsection{K-Segment Model}
%Lastly, we look at the regime where know the number of actions that take place but not the ordering. This could be used in applications where the same actions are happening but sometimes in different orders. We solve the problem $Y=\argmax_Y E(X,Y) \text{ s.t .}  |\mathbb{Y}| = K$. Again, this can be computed using dynamic programming and is described in Algorithm~\ref{alg:KSegment}.

%\begin{algorithm}[tb]
% \caption{Forward pass for decoding when we have a known task model}
%\KwData{$X$: features, $S$: action sequence}
%%\KwResult{$Y: \text{frame-wise labels}$}
%$V \in \mathbb{R}^{T \times |S| } $\;
%$V_{t,k} = -\infty$\;
%\For{$k=1:|S|$}{
%	\For{$t=1:T$}{
%		$v_{prev} = V_{t-1,k-1} + w^T \Psi(X, S_k, S_{k-1}, t)$\;
%		$v_{curr} = V_{t-1, k} + w^T \Psi(X, S_k, S_k, t)$ \;
%		$V_{t,k} =\max(v_{prev}, v_{curr})$\;
%	}
%}
% \label{alg:Inference}
%\end{algorithm}  



%\subsubsection{Online inference}
%For each of the aforementioned inference methods the score is simply a function of the previous data. Thus we can easily modify our previous methods to be computed in an online fashion. Instead of backtracking from $T$ to $1$ we backtrack from time $t$ to $1$ to find the best sequence so far. Note that in the case where we have a task model there is uncertainty in which segment (from $k=1...K$) is being performed at time $t$. To account for this we maximize over all segments: $k_t = \argmax_k V_{t,k}$. 
%%Online inference finds the best sequence given the data from 
%%Similarly in regime 3 we maximize over both the segment number and the class: $Y_t = \argmax_{k,y} V_{t,k,y}$.


%\subsubsection{Filtering}
%One caveat to using a frame-wise inference method, like Viterbi, is that it operates on a frame-by-frame basis. Coupled with our skip frame transition features we find it prone to over- or under- segmentation issues; while these features provide valuable information about action transitions, they occasionally oscillate between states along what should be long contiguous segments. To reduce this issue we simply apply a median filter to the predictions in the traditional inference regime. 

%While the Viterbi algorithm finds the optimal action label for each frame, if the features are very noisy it is common for this method to severely oversegment the data, as shown in figure~\ref{fig:predictions}. This is largely due to the skip-frame transitions from the SC-CRF; they provide valuable information about action transitions, however there tends to be oscillations they do not tend to stay consistent 

%While the pairwise transition term in our model should penalize inconsistent action transitions, it does not penalize the model from transitioning too frequently.



%\begin{align}
%S = \argmax\limits_{S_1,\dots, S_M} E(s, S)\\
%s.t. \sum_{i=1}^M d_i = T \nonumber \\
% M \leq K \nonumber
%\end{align}
%%Y = \arg\max\limits_{Y, M} E(s, S)\\
%%s.t. M \leq K
%
%\begin{align}
%Y = \arg\max\limits_{M \leq K} \max\limits_{S_1,\dots, S_M} E(s, S)\\
%s.t. \sum_{i=1}^M d_i = T
%\end{align}


==> sections/old_related_work.tex <==
\section{Related Work}
\label{sec:related}

Linear chain models like Hidden Markov Models (HMMs) have been a mainstay for modeling timeseries data since the late 1980s \cite{Rabiner1989} due to their simplicity and effectiveness in a broad range of applications. More recently, models like Conditional Random Fields (CRFs) \cite{Lafferty2001} and Max Margin Markov Networks \cite{Taskar2003} have improved the accuracy of linear chain models by removing the assumption that data at each timestep must be independent. In this proposal I build upon CRFs due to their ease of use in terms of encoding relationships between data and corresponding labels as well as their widespread use. 
While traditionally these models were learned using probabilistic approaches, over the past decade it has become common to use the Structural Support Vector Machine formulation for learning parameters. Some methods for learning include subgradient descent \cite{Shor_1985}, cutting planes \cite{Tsochantaridis2005}, and Block  Coordinate Frank Wolfe Structural \cite{lacoste-julien_icml_2013}. See \cite{Sutton2006} for a general overview of CRFs and \cite{Nowozin2010} for a more recent vision-oriented overview that also discusses Structural SVMs. Mueller et al. has a nice comparison of speed and accuracy of recent optimization algorithms as applied to semantic segmentation \cite{Muller2013a,mueller_jmlr_2014}.

\TODO{RNNs section! argue why they aren't better here. could also do a comparison (using TStruct or Keras)} much of this can be generalized to RNNs. however, in that case we have latent variables. that makes a lot of sense in areas like NLP where the features (patterns/signals/tokenization) is good. However, in our applications we are struggling to get good signal. Maybe mention closing parenthesis thing. Can be handled by RNN but not by mine… but we don’t really care about this because we can’t even do simple things. 


Other frame-based linear chain models have also been developed including Hidden Semi Markov Models \cite{Yu2010}, Coupled Hidden Semi Markov Models \cite{Natarajan2007}, and Max-Margin Hidden Conditional Random Fields \cite{Mori2009}. Both \cite{Natarajan2007} and \cite{Mori2009} were developed for human action recognition. 

In my work I use a Semi Markov Conditional Random Field (SM-CRF) for joint segmentation and recognition of activities.
This model was first proposed by Sarawagi and Cohen~\cite{sarawagi_nips_2004} for the Named Entity Recognition problem in Natural Language Processing. 
%Their Semi Markov component captures entities composed of multiple words. 
More recently it has been used for activity recognition in the computer vision and sensing communities~\cite{pirsiavash_cvpr_2014,hu_icra_2014,van_jaise_2010,lee_ai_2011,tao_miccai_2013,shi_ijcv_2011,tang_cvpr_2012}. 
%While the Semi Markov Model typically increases the accuracy compared to a linear chain model, many of these approaches use energy functions that are not submodular. In *****. 
Shi \textit{et al.}~\cite{shi_ijcv_2011} use a discriminative Semi Markov model with a histogram of cuboid and shape context features to recognize single actions in the KTH and CMU MoBo datasets. They also evaluate their model on a simple activity dataset they generated that includes the actions ``walking," ``bending," and ``drawing."
The structured model of Pirsiavash and Ramanan~\cite{pirsiavash_cvpr_2014} is similar to mine.
They propose a segmental regular grammar for decomposing actions into latent action primitives. This model can be viewed as a latent Semi Markov CRF if the objective is used as the energy in a Gibbs distribution.
Their representation is a set of normalized histograms using Dense Trajectories and other local video features.
Also relevant is the model employed by Hu \textit{et al.}~\cite{hu_icra_2014}, %is also related to our work. They
which uses a latent Conditional Random Field where nodes correspond to the data, actions, and action primitives.
%They perform inference in their loopy graph efficiently by collapsing the latent variable to make the graph a linear chain.
%They then treat their model as a Semi Markov Model where the state space is a product of their latent and action states.
%\Chris{Removed some sentences on Hu I thought looked unnecessary; you might want to add them back in.}

Other models for structured prediction include Markov Logic Networks, Dynamic Bayes Nets, and other variations on Conditional Random Fields. 
Morariu and David~\cite{morariu_cvpr_2011} create segmentation hypotheses using Allen's Interval Logic with Markov Logic Networks to recognize fine grained activities in 1-vs-1 basketball games. They define a set of domain-specific features to capture relationships between the players and the environment.
Vo \textit{et al.}~\cite{vo_cvpr_2014} assume there exists a known task model  represented as a Context Free Grammar. %They convert this grammar into a Sequential Interval Network, a special case of a Dynamic Bayes Network.
Their features are based on detected hand positions, a set of known bin locations, and duration. Koppula and Saxena~\cite{koppula_icml_2013} propose a CRF model that captures six potentials, like object-object and action-object interactions, for activity recognition of household tasks. Action segmentation is performed by sampling and evaluating many different graph structures. 

----------- 
Add Minh, other SM-CRF papers

Semi-Markov Conditional Random Field with High-Order Features
%http://www.comp.nus.edu.sg/~yenan/pub/crf-icmlw11.pdf

Probabilistic versus discriminative

actions in vision

actions in other timeseries (e.g. robotics)

touch on speech?

segmental models

THUMOS



==> sections/related_work_b.tex <==
\section{Related Work}

Recently there have been a large number applications for fine-grained action recognition in the domains of cooking~\cite{rohrbach_cvpr_2012, lei_ubicomp_2012,ramirez_iros_2014,ubicomp_2014}, sports analysis~\cite{morariu_cvpr_2011, pirsiavash_cvpr_2014}, human-robot assembly~\cite{vo_cvpr_2014,vo_icra_2014}, and activities of daily living~\cite{koppula_icml_2013,otherCADpaper_icra_2014}.


\label{sec:related}
\hspace{5pt}\\
% ------------------------------------------------------------------------------------
\textbf{Framewise Models}:
Linear chain models like Hidden Markov Models (HMMs) have been a mainstay for modeling timeseries data since the late 1980s \cite{Rabiner1989} due to their simplicity and effectiveness in a broad range of applications. Since the early 2000s models like Conditional Random Fields (CRFs) \cite{Lafferty2001} and Max Margin Markov Networks \cite{Taskar2003} have become commonplace due to their relaxed independence assumptions and often improved accuracy. Recently there has been a resurgence of Recurrent Neural Networks (RNNs) for modeling timeseries sequences \cite{?,?}. These are similar to a Linear Chain CRF but add a layer of continuous latent variables. 

The speech recognition community (e.g. \cite{Ng-DeepSpeech}) has started to look at adding convolutional layers into RNNs.
This is similar to our work except that they learn a set of shared convolutional filters common among all classes while our filters are learned for each individual action. This allows us to learn what features (e.g. objects usage) are dominant for each action and how these features transition. For example, in a cutting action we see our filters learn that a user picks up a knife, uses it, and sets it down.
%Typically a CNN or RNN learns a hierarchy of filters that are shared between different classes. This means that filter \#1 may be used to model both \textit{cutting} and \textit{peeling}. In addition the filters are applied hierarchically such that convolutions are applied to the output of other convolutions. While it is possible that this approach achieves high performance in our application using these black box methods, they do not learn a set of interpretable action primitives. In our work we model each action as a small, independent set of filters which we learn using a Latent Structural Support Vector Machine.
%
\\
\\
\textbf{Segmental Models}: Many of the recent papers in fine-grained action recognition have introduced new structured models~\cite{koppula_icml_2013,vo_cvpr_2014,vo_icra_2014,yezhou_aaai_2015, hu_icra_2014,morariu_cvpr_2011,pirsiavash_cvpr_2014,hu_icra_2014,van_jaise_2010,lee_ai_2011,
tao_miccai_2013,shi_ijcv_2011,tang_cvpr_2012}. Koppula and Saxena~\cite{koppula_icml_2013} propose a CRF model that captures six interactions -- such as between different objects, and between actions and objects -- for activity recognition of household tasks. These interactions are defined between different temporal segments. These segments are generated by sampling and evaluating many different graph structures. Vo and Bobick \cite{vo_cvpr_2014} introduce the Sequential Interval Network which takes a task model in the form of a Context Free Grammar and converts it into a Dynamic Bayes Network. They apply it to a toy assembly task dataset and in \cite{vo_icra_2014} apply it to human robotic interaction. Their features are based on detected hand positions, a set of known bin locations, and duration. Yezhou et al \cite{yezhou_aaai_2015} use a probabilistic manipulation-action grammar to recognize sequences of cooking tasks in unconstrained videos. Their features are object and hand grasp-types detected with a deep network. In each of these cases the features are defined individually per frame or on the statistics of a segment. In our work we look at developing a richer representation of how features change over time.
%
\\
\\
\textbf{Handcrafted features}: Ramirez-Amaro et al \cite{Ramirez-Amaro_iros_2014} claim that complicated temporal models are unnecessary in situations where the features are highly accurate. They look at two cooking tasks in a setup where they can easily detect relevant objects and the hands of a user. They use semantic reasoning (via a decision tree) with simple predicates like \textit{hand\_moving} and  \textit{object\_in\_hand} to classify fine-grained cooking actions. While their claim may be true in specific applications, contrary to our approach, their method may not work well in domains where there is high variability in features.
Similarly, Yezhou et al~\cite{Yezhou_cvpr_2014,Yezhou_iros_2014} learn how objects change as a function of actions. For example, in a cutting task they model the transition from a whole cucumber to two halves as a change from one segment to two. Again, while this work provides interesting insights into action-object relationships, it does not easily generalize to new object-types or features.
%
%Morariu and Davis~\cite{morariu_cvpr_2011} generate segmentation hypotheses %using Allen's Interval Logic and 
%evaluate with Markov Logic Networks to recognize actions in one-vs-one basketball games. They define a set of domain-specific features to capture relationships between the players and the environment.
%
%Also relevant is the model employed by Hu \textit{et al.}~\cite{hu_icra_2014}, which uses a latent Conditional Random Field where nodes correspond to the data, actions, and action primitives. They perform inference in their loopy graph efficiently by collapsing the latent variable to make the graph a linear chain.
%
% ------------------------------------------------------------------------------------
%\\
%\\
%\textbf{Large scale action recognition}:
%Related work in the computer vision community has primarily focused on large-scale action recognition where the goal is to classify whether a Youtube-style video contains a high level activity like \textit{surfing} or \textit{skiing}. While there have been many papers developing new feature representations (e.g. Dense Trajectories) \cite{wang_iccv_2011,wang_iccv_2013,?}, we have found they do not perform well for fine-grained action recognition. 
%This was also found by participants of the 2015 THUMOS action recognition and localization challenge \cite{THUMOS}. Thus, despite recent progress, these methods tend not to be suitable for robotics.
\TODO{Add paragraph for Fox-ubicomp. and Dundee}


%\textbf{Semi-Markov Models}:
%More recently it \TODO{SM-CRF} has been used for activity recognition in the computer vision communities~\cite{pirsiavash_cvpr_2014,hu_icra_2014,van_jaise_2010,lee_ai_2011,tao_miccai_2013,shi_ijcv_2011,tang_cvpr_2012}. 
%%While the Semi Markov Model typically increases the accuracy compared to a linear chain model, many of these approaches use energy functions that are not submodular. In *****. 
%Shi \textit{et al.}~\cite{shi_ijcv_2011} use a discriminative Semi Markov model with a histogram of cuboid and shape context features to recognize single actions in the KTH and CMU MoBo datasets. They also evaluate their model on a simple activity dataset they generated that includes the actions ``walking," ``bending," and ``drawing."
%Pirsiavash and Ramanan~\cite{pirsiavash_cvpr_2014} propose a segmental regular grammar for decomposing actions into latent action primitives. This model can be viewed as a latent Semi Markov CRF if the objective is used as the energy in a Gibbs distribution.
%Their representation is a set of normalized histograms using Dense Trajectories and other local video features.



%\TODO{Where to include linear dynamical / hybrid systems}




==> sections/related_work_nov2.tex <==
\section{Related Work}
\label{sec:related}


To contrast, most action recognition papers (e.g. \cite{?,?,?}) classify individual video clips  (typically with short duration) with a single action label.  In large scale recognition the labels tend to be very disparate. For example UCF 101~\cite{UCF} includes classes like \textit{Applying Makeup} and \textit{Archery}. Techniques that perform well on large scale datasets tend to use holistic features with bag of words type models which capture statistics on complete clips as opposed to fine-grained segments. 

\textbf{Comparison with robotics/sensing} Many others have explored this problem from the robotics setting where it is common to record other sensing modalities along with video. Both datasets we use come from this setting and thus we compare out results against a variation of our model using these signals. 50 Salads contains a set of 10 accelerometers and a set of 

Space: Status quo: IDT+FV. Captures info that is way too local. Ignores Cartesian information which is useful in many problems (more broadly object relationships). Our approach: ST-CNN. As shown in [Zisserman; 2 streams] a spatial cnn with RGB and Optical flow captures very similar information to IDT but also captures spatial information.

Time: Status quo: sliding window; RNN+LSTM. These don't explicitly model how features transition throughout time. LSTM uninterpretable. HMMs too local. 

\textbf{Feature representations:} 
IDT. lots of e.g.s. GO THROUGH MPII CLASSIFICATION PAPERS. trecvid?
\\
\textbf{Large scale action recognition}:
Related work in the computer vision community has primarily focused on large-scale action recognition where the goal is to classify whether a Youtube-style video contains a high level activity like \textit{surfing} or \textit{skiing}. While there have been many papers developing new feature representations (e.g. Dense Trajectories) \cite{wang_iccv_2011,wang_iccv_2013,?}, we have found they do not perform well for fine-grained action recognition. 
This was also found by participants of the 2015 THUMOS action recognition and localization challenge \cite{THUMOS}. Thus, despite recent progress, these methods tend not to be suitable for robotics.

%Copious work has been done in the AI and robotics communities to model how the state of the world (e.g. the location of a plate) changes as a function of an action being performed (e.g. \textit{put\_plate\_on\_table}) \cite{AskChris}. These researchers have been using models like STRIPS \cite{Nilson?} for task modeling since the 1970s. However, due to limitations in perception, computer vision systems often rely on using Bag of Words or Fisher Vector-esque representations. These features correspond to statistics of image patches instead of meaningful object relationships. 
Despite a significant amount of research in this area there is a dearth of work focused on fine-grained recognition. Most papers target large-scale action recognition where the goal is to classify whether a Youtube-style video contains a high level activity like \textit{surfing} or \textit{skiing}. 
%We argue that applications for fine-grained recognition require a different set of features and a different variety of models. In these settings we seek to model how the scene varies over the course of an activity -- whereas most models capture high level contextual information (e.g. a mountainous background versus basketball arena) which tends not to change much within an environment.
\\
\textbf{CNNs: Speech, language, vision} 
\\
\\
%Recently there have been a large number applications for fine-grained action recognition in the domains of cooking~\cite{rohrbach_cvpr_2012, lei_ubicomp_2012,ramirez_iros_2014,ubicomp_2014}, sports analysis~\cite{morariu_cvpr_2011, pirsiavash_cvpr_2014}, human-robot assembly~\cite{vo_cvpr_2014,vo_icra_2014}, and activities of daily living~\cite{koppula_icml_2013,otherCADpaper_icra_2014}.
%\hspace{5pt}\\
% ------------------------------------------------------------------------------------
%\textbf{Framewise Models}:
%Linear chain models like Hidden Markov Models (HMMs) have been a mainstay for modeling timeseries data since the late 1980s \cite{Rabiner1989} due to their simplicity and effectiveness in a broad range of applications. Since the early 2000s models like Conditional Random Fields (CRFs) \cite{Lafferty2001} and Max Margin Markov Networks \cite{Taskar2003} have become commonplace due to their relaxed independence assumptions and often improved accuracy. Recently there has been a resurgence of Recurrent Neural Networks (RNNs) for modeling timeseries sequences \cite{?,?}. These are similar to a Linear Chain CRF but add a layer of continuous latent variables. 
%
%The speech recognition community (e.g. \cite{Ng-DeepSpeech}) has started to look at adding convolutional layers into RNNs.
%This is similar to our work except that they learn a set of shared convolutional filters common among all classes while our filters are learned for each individual action. This allows us to learn what features (e.g. objects usage) are dominant for each action and how these features transition. For example, in a cutting action we see our filters learn that a user picks up a knife, uses it, and sets it down.
%
%Typically a CNN or RNN learns a hierarchy of filters that are shared between different classes. This means that filter \#1 may be used to model both \textit{cutting} and \textit{peeling}. In addition the filters are applied hierarchically such that convolutions are applied to the output of other convolutions. While it is possible that this approach achieves high performance in our application using these black box methods, they do not learn a set of interpretable action primitives. In our work we model each action as a small, independent set of filters which we learn using a Latent Structural Support Vector Machine.
%
\\
\\
\textbf{Segmental Models}: 
Several recent papers have used a semi-Markov assumption to jointly segment and recognize actions~\cite{pirsiavash_cvpr_2014,shi_ijcv_2011,hu_icra_2014,van_jaise_2010,lee_ai_2011,tao_miccai_2013tang_cvpr_2012}. 
%There are two primary benefits to using this assumption.
Semi-Markov models assume that the action label of a segment depends on the action label of the previous segment.
This is contrary to traditional Markov models 
which assume that every action label depends on the label of the previous frame, often as little as 33 milliseconds earlier.
Shi \textit{et al.}~\cite{shi_ijcv_2011} use a discriminative Semi Markov model with a histogram of cuboid and shape context features to recognize single actions in the KTH and CMU MoBo datasets. They also evaluate their model on a simple activity dataset they generated that includes the actions ``walking," ``bending," and ``drawing."
Pirsiavash and Ramanan~\cite{pirsiavash_cvpr_2014} propose a segmental regular grammar for decomposing actions into latent action primitives. This model can be viewed as a latent Semi Markov CRF if the objective is used as the energy in a Gibbs distribution.
Their representation is a set of normalized histograms using Dense Trajectories and other local video features.

%Typically, in our setting Markov models have a high self-transition probability which has the effect of smoothing the data.
%When such models are applied to data with long segments wherein that many adjacent frames have the same label, they learn a high self-transition probability which has the effect of smoothing the data.
%This implies that semi-Markov models are better at encoding important higher-level contextual information than Markov models.
%This assumption implies that an action, a segment of data perhaps on the order of a few seconds, is dependent only on the previous action. 


%\textbf{Semi-Markov Models}:
%More recently it \TODO{SM-CRF} has been used for activity recognition in the computer vision communities~\cite{pirsiavash_cvpr_2014,hu_icra_2014,van_jaise_2010,lee_ai_2011,tao_miccai_2013,shi_ijcv_2011,tang_cvpr_2012}. 
%While the Semi Markov Model typically increases the accuracy compared to a linear chain model, many of these approaches use energy functions that are not submodular. 


Many of the recent papers in fine-grained action recognition have introduced new structured models~\cite{koppula_icml_2013,vo_cvpr_2014,vo_icra_2014,yezhou_aaai_2015, hu_icra_2014,morariu_cvpr_2011,pirsiavash_cvpr_2014,hu_icra_2014,van_jaise_2010,lee_ai_2011,
tao_miccai_2013,shi_ijcv_2011,tang_cvpr_2012}. Koppula and Saxena~\cite{koppula_icml_2013} propose a CRF model that captures six interactions -- such as between different objects, and between actions and objects -- for activity recognition of household tasks. These interactions are defined between different temporal segments. These segments are generated by sampling and evaluating many different graph structures. Vo and Bobick \cite{vo_cvpr_2014} introduce the Sequential Interval Network which takes a task model in the form of a Context Free Grammar and converts it into a Dynamic Bayes Network. They apply it to a toy assembly task dataset and in \cite{vo_icra_2014} apply it to human robotic interaction. Their features are based on detected hand positions, a set of known bin locations, and duration. Yezhou et al \cite{yezhou_aaai_2015} use a probabilistic manipulation-action grammar to recognize sequences of cooking tasks in unconstrained videos. Their features are object and hand grasp-types detected with a deep network. In each of these cases the features are defined individually per frame or on the statistics of a segment. In our work we look at developing a richer representation of how features change over time.
%
\\
\\
\textbf{Robotics / Handcrafted features}: Ramirez-Amaro et al \cite{Ramirez-Amaro_iros_2014} claim that complicated temporal models are unnecessary in situations where the features are highly accurate. They look at two cooking tasks in a setup where they can easily detect relevant objects and the hands of a user. They use semantic reasoning (via a decision tree) with simple predicates like \textit{hand\_moving} and  \textit{object\_in\_hand} to classify fine-grained cooking actions. While their claim may be true in specific applications, contrary to our approach, their method may not work well in domains where there is high variability in features.
Similarly, Yezhou et al~\cite{Yezhou_cvpr_2014,Yezhou_iros_2014} learn how objects change as a function of actions. For example, in a cutting task they model the transition from a whole cucumber to two halves as a change from one segment to two. Again, while this work provides interesting insights into action-object relationships, it does not easily generalize to new object-types or features.
%
%Morariu and Davis~\cite{morariu_cvpr_2011} generate segmentation hypotheses %using Allen's Interval Logic and 
%evaluate with Markov Logic Networks to recognize actions in one-vs-one basketball games. They define a set of domain-specific features to capture relationships between the players and the environment.
%
%Also relevant is the model employed by Hu \textit{et al.}~\cite{hu_icra_2014}, which uses a latent Conditional Random Field where nodes correspond to the data, actions, and action primitives. They perform inference in their loopy graph efficiently by collapsing the latent variable to make the graph a linear chain.
%
% ------------------------------------------------------------------------------------
%\\
%\\


\THOUGHT{mention pose-based methods?}
\THOUGHT{mention object proposals somewhere? future work?}


==> sections/segmental_models.tex <==
\section{Segmental Models}
\label{sec:segmental}

Let us define a Segmental Model (SM) as depicted in figure~\ref{fig:models}. The probabilistic version of this model is similar to a Semi-Markov Conditional Random Field~\cite{sarawagi_nips_2004}. Let the variable, $X_t$, be a set of features at time $t$ and tuple $S_j=(y_j, s_j, d_j)$ be the $j$th fine-grained action segment where $y_j$ is the action label, $s_j$ is the start time, and $d_j$ is the segment duration. There are an arbitrary number of segments, $M$, in any video such that $S=[S_1...S_M]$. Given the data $X$ we seek to find the labels $S$ that maximize our energy function $E(X,S)$. Now we define our energy over all segments instead of timesteps:
\begin{align}
	E(X,S) = \sum_{j=1}^M \sum_{j=1}^P w_i^T \phi_i(X, S)
\end{align}
 
Again, we learn the parameters of our model using the Structural Support Vector Machine. However, now we will experiment with different loss functions. 

One important issue with frame-wise models is that there is no local consistency -- it is common for predicted actions to change more erratically than with a segmental model. This is true both for the potentials and with the loss function. Here we introduce a loss function that helps ensure local consistency. 

If we know the association of each segment $S_j$ in the ground truth labels $Y^*$ and the corresponding segments in an arbitrary other labeling $Y$ we can use an overlap metric to determine how correct the labeling is. Here we use the intersection over union loss function where $|S_j|$ denotes the length of a segment:
\begin{align}
\Delta(Y^*, Y) = \sum_{j=1}^M \frac{|S^*_j \cap S_j |}{|S^*_j \cup S_j |}
\end{align}

However, during inference it is common to have a different number of segments in each labeling. Thus we have to simplify this to a function over the ground truth segments:
\begin{align}
\Delta(Y^*, Y) = \sum_{j=1}^M \frac{|y_t \in S^*_j|}{|S^*_j|}
\end{align}
This represents the fraction of predicted labels that have the same class as the truth labels. \TODO{is this any different than a slightly modified Hamming function where the loss is now a sum over segments instead of frames?}.


%\subsection{Inference}
%\label{sec:inference}

%\begin{align}
%\label{eq:sm_inference}
%V(y, t) = \max\limits_{\substack{d=1...D \\ y_{t-d}}} V(y_{t-d}, t-d) + w^T  \Phi(X_{t-d:t}, y, y_{t-d})
%\end{align}

%\begin{tabular}{c}
%\begin{align}
%
%C_{DM}(X, y=c) = \sum_{j=1}^M \frac{1}{d} \sum_{t=s_j}^{s_j+d_j} X_t \cdot \mathbf{1}[y_j=c]
%\end{align}
%\caption{Table of Equations}
%\label{table:sm_eqns}
%\end{tabular}

%\begin{figure}
%\center
%\begin{tabular}{|l|}
%\hline
%\textbf{Segmental terms}\\
%$C_{DM}(X, y=c) = \frac{1}{d_j} \sum_{t=s_j}^{s_j+d_j} X_t \cdot \mathbf{1}[y_j=c]$ \\
%$C_{FM}(X, y=c) = X_t \cdot \mathbf{1}[y_j=c]$ \\
%\hline
%\end{tabular}\caption{List of Energy Potentials}
%\label{table:sm_eqns}
%\end{figure}

\subsection{Potentials}
In this section we describe three types of potentials: segmental functions and duration functions. The pairwise and priors can be applied in a straightforward manner so we gloss over these for brevity.
The segmental pairwise class potential is similar to the framewise variant except that we model the transitions between sequential segments instead of between sequential frames. The temporal priors are now applied over each segment instead of each frame.

% we do not Note that the priors we discussed in the previous section can be generalized to the segmental model in a straightforward fashion. Thus, we choose to skip over those here. 


\textbf{Data Statistics Potential}
Mean function:
\begin{align}
C_{DM}(X, y=c) = \frac{1}{d_j} \sum_{t=s_j}^{s_j+d_j} X_t \cdot \mathbf{1}[y_j=c]
\end{align}

%\subsubsection{Bag of Words Potential}
%\begin{align}
%C_{DM}(X, y=c) = \sum_{j=1}^M \frac{1}{d} \sum_{t=s_j}^{s_j+d_j} X_t \cdot \mathbf{1}[y_j=c]
%\end{align}

\textbf{Fixed-time Template Model}
\begin{align}
C_{FT}(X, y=c) = \sum_{j=1}^M X_{s_j:s_j+d_j} \cdot \mathbf{1}[y_j=c]
\end{align}



%\subsubsection{Edge-transition Template Model}

\subsection{Duration models}
Discrete
\begin{align}
C_{DD}(X, S) = d_j
\end{align}

Quadratic
\begin{align}
C_{DQ}(X, S) = [d_j, d_j^2]
\end{align}

%\subsection{Pairwise Potentials}

%Frame-wise, segment-wise

%\subsubsection{Pairwise Class Potential}
%The segmental pairwise class potential is similar to the framewise variant except that we model the transitions between sequential segments instead of between sequential frames.
%
%This cost is modeled as:
%\begin{align}
%C_{sp}(X, S) = \sum_{t=j}^M \mathbf{1}[y_{j-1}=c_1,y_j=c_2]
%\end{align}

\subsection{Submodularity}
\TODO{point to Hoai somewhere here}
Note that we must take more care in defining our potentials in the segmental model. Because we are maximizing over different segment lengths we must worry about adding too much bias towards lengths that are too short or long. As we describe below, it is easy to accidentally oversegment the data. Recall $d$ is the segment duration and $y'$ is the previous label. Let us assume our only potential is the mean data potential: $\phi (X, y, s, d) = \frac{1}{d} \sum_{t=s}^{s+d} X_t$.


\TODO{fix weights}
\begin{align}
	V(j, y, s, d) = \arg\max_{y', d} \sum_{=1}^P \phi_i (X, y, s, d, y') \\
	V(j, y, s, d) = \arg\max_{y, d} w_y^T \frac{1}{d} \sum_{t=s}^{s+d} X_t
\end{align}

Now let us look at two special cases where $d=1$ and $d=2$:
\begin{align}
	V(j, y, s; d=1) =  w_y^T X_s \\
	V(j, y, s; d=2) = w_y^T \frac{1}{2} \sum_{t=s}^{s+1} X_t
\end{align}

If we the data is constant through times $t$ to $t+d'$ then the model will oversegment the data: $V(j, y, s; d=1)=V(j, y, s; d=d')$! Our goal is to segment the data into a minimal, non-repeating action primitives. Thus, we must take care with choosing our potentials. In fact, we tend to find that normalized functions are not great potentials. Some examples include the mean potential and histogram potential. Note that this extends beyond simple constant data as well. For a more in-depth example see Appendix~\ref{sec:appendix}.

While this may seem obvious, there are several prior papers that use this potential \cite{}. There are other ways of going around this -- for example, by setting the self-transition weights in a pairwise transition matrix to negative infinity -- however, they simply ignore the core modeling issue. 

\subsection{Learning}
\TODO{should I make a new section for this?}

Q: Can any loss function be used in the SSVM?\\
A: No, the loss function should be \textit{decomposable} over the input frames. While the common Hamming loss is not the best way for modeling loss (e.g. it does not penalize for oversegmenting the data into lots of noisy labels) \cite{SSVM decomposable papers}

Q: What are some common loss functions\\
A: Hamming, overlap (Intersection over union), transition cost \cite{pirsiavash_cvpr_2014}, ?

Q: What effect does he loss function have on the segmental model?

Q: How can I interpret loss augmented inference\\
A: Loss augmented inference is used to find the best (mostly) incorrect prediction given the current data and ground truth labels. 

Q: Why is the SSVM with Hamming loss bad for segmental models?\\
A: At each iteration of learning our model weights are updated based solely on a specific set of true positives and false positives. Recall, the SSVM uses loss augmented inference to find the best scoring (mostly) incorrect predictions. This set of predictions is chosen by $\hat{y} = max_y \Delta(\hat{y}, y^*) + w^T (\Phi(X, \hat{y}) - \Phi(X, y^*))$. In a segmental model we expect there are contiguous blocks of data that are labeled with the same class (e.g. all frames from time 1 to 10 are of walking). However, the Hamming loss is a function over each individual frame as opposed to a segment of frames. Thus is possible (and in common in practice) for a series of consecutive frames to have a mixture of labels. This is especially important when we are trying to learn the parameters of a duration potential. 

What if we had a different loss for different weights?\\
This seems like a reasonable idea. This cannot be done with the current SSVM objective. However, you could learn the weights independently for each potential where a different loss function is used for each. This is sometimes referred to as pretraining. You can then learn a set of weights that learn the importance of each term to combine them together. 

Q: What is the impact of using different regularizers on the SSVM objective?\\
A: We experimented with the common SSVM formulation (using the $||w||_2$ regularizer) as well as variants with a $||w||_1$ regularizer, a $||w||_*$ regularizer, and without any regularizer. In our findings there was little difference in the accuracy of our results on the JIGSAWS dataset.

Q: What is the effect of the norms of each of the weights of the potential functions?

